Plant species richness prediction from DESIS hyperspectral data: A comparison study on feature extraction procedures and regression models

The diversity of terrestrial vascular plants plays a key role in maintaining the stability and productivity of ecosystems. Airborne hyperspectral imaging has shown promise for measuring plant diversity remotely, but to operationalise these efforts over large regions we need to advance satellite-based alternatives. The advanced spectral and spatial specification of the recently launched DESIS (the DLR Earth Sensing Imaging Spectrometer) instrument provides a unique opportunity to test the potential for monitoring plant species diversity with spaceborne hyperspectral data. This study provides a quantitative assessment on the ability of DESIS hyperspectral data for predicting plant species richness in two different habitat types in southeast Australia. Spectral features were first extracted from the DESIS spectra, then regressed against on-ground estimates of plant species richness, with a two-fold cross validation scheme to assess the predictive performance. We tested and compared the effectiveness of Principal Component Analysis (PCA), Canonical Correlation Analysis (CCA), and Partial Least Squares analysis (PLS) for feature extraction, and Kernel Ridge Regression (KRR), Gaussian Process Regression (GPR), and Random Forest Regression (RFR) for species richness prediction. The best prediction results were $r=0.76$ and $\text{RMSE}=5.89$ for the Southern Tablelands region, and $r=0.68$ and $\text{RMSE}=5.95$ for the Snowy Mountains region. Relative importance analysis for the DESIS spectral bands showed that the red-edge, red, and blue spectral regions were more important for predicting plant species richness than the green bands and the near-infrared bands beyond red-edge. We also found that the DESIS hyperspectral data performed better than Sentinel-2 multispectral data in the prediction of plant species richness.

==> Definitions/journalnames.tex <==
%%Updated on 15 January 2022
%,% Website Name,%,%,% Website Name,%%,% Full Name,%%,% Short Name,%%,% DOI abbr,%%,% ISSN,% \continuouspages
%\DeclareOption{}{\gdef\@journal{}\gdef\@journalfull{}\gdef\@journalshort{}\gdef\@doiabbr{}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{acoustics}{\gdef\@journal{acoustics}\gdef\@journalfull{Acoustics}\gdef\@journalshort{Acoustics}\gdef\@doiabbr{acoustics}\gdef\@ISSN{2624-599X}\gdef\@continuouspages{yes}}
\DeclareOption{actuators}{\gdef\@journal{actuators}\gdef\@journalfull{Actuators}\gdef\@journalshort{Actuators}\gdef\@doiabbr{act}\gdef\@ISSN{2076-0825}}
\DeclareOption{addictions}{\gdef\@journal{addictions}\gdef\@journalfull{Addictions}\gdef\@journalshort{Addictions}\gdef\@doiabbr{}\gdef\@ISSN{0006-0006}}
\DeclareOption{admsci}{\gdef\@journal{admsci}\gdef\@journalfull{Administrative Sciences}\gdef\@journalshort{Adm. Sci.}\gdef\@doiabbr{admsci}\gdef\@ISSN{2076-3387}}
\DeclareOption{adolescents}{\gdef\@journal{adolescents}\gdef\@journalfull{Adolescents}\gdef\@journalshort{Adolescents}\gdef\@doiabbr{adolescents}\gdef\@ISSN{2673-7051}\gdef\@continuouspages{yes}}
\DeclareOption{aerospace}{\gdef\@journal{aerospace}\gdef\@journalfull{Aerospace}\gdef\@journalshort{Aerospace}\gdef\@doiabbr{aerospace}\gdef\@ISSN{2226-4310}}
\DeclareOption{agriculture}{\gdef\@journal{agriculture}\gdef\@journalfull{Agriculture}\gdef\@journalshort{Agriculture}\gdef\@doiabbr{agriculture}\gdef\@ISSN{2077-0472}}
\DeclareOption{agriengineering}{\gdef\@journal{agriengineering}\gdef\@journalfull{AgriEngineering}\gdef\@journalshort{AgriEngineering}\gdef\@doiabbr{agriengineering}\gdef\@ISSN{2624-7402}\gdef\@continuouspages{yes}}
\DeclareOption{agrochemicals}{\gdef\@journal{agrochemicals}\gdef\@journalfull{Agrochemicals}\gdef\@journalshort{Agrochemicals}\gdef\@doiabbr{agrochemicals}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{agronomy}{\gdef\@journal{agronomy}\gdef\@journalfull{Agronomy}\gdef\@journalshort{Agronomy}\gdef\@doiabbr{agronomy}\gdef\@ISSN{2073-4395}}
\DeclareOption{ai}{\gdef\@journal{ai}\gdef\@journalfull{AI}\gdef\@journalshort{AI}\gdef\@doiabbr{ai}\gdef\@ISSN{2673-2688}\gdef\@continuouspages{yes}}
\DeclareOption{algorithms}{\gdef\@journal{algorithms}\gdef\@journalfull{Algorithms}\gdef\@journalshort{Algorithms}\gdef\@doiabbr{a}\gdef\@ISSN{1999-4893}}
\DeclareOption{allergies}{\gdef\@journal{allergies}\gdef\@journalfull{Allergies}\gdef\@journalshort{Allergies}\gdef\@doiabbr{allergies}\gdef\@ISSN{2313-5786}}
\DeclareOption{alloys}{\gdef\@journal{alloys}\gdef\@journalfull{Alloys}\gdef\@journalshort{Alloys}\gdef\@doiabbr{alloys}\gdef\@ISSN{2674-063X}\gdef\@continuouspages{yes}}
\DeclareOption{analytica}{\gdef\@journal{analytica}\gdef\@journalfull{Analytica}\gdef\@journalshort{Analytica}\gdef\@doiabbr{analytica}\gdef\@ISSN{2673-4532}\gdef\@continuouspages{yes}}
\DeclareOption{analytics}{\gdef\@journal{analytics}\gdef\@journalfull{Analytics}\gdef\@journalshort{Analytics}\gdef\@doiabbr{analytics}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{anatomia}{\gdef\@journal{anatomia}\gdef\@journalfull{Anatomia}\gdef\@journalshort{Anatomia}\gdef\@doiabbr{anatomia}\gdef\@ISSN{2813-0545}\gdef\@continuouspages{yes}}
\DeclareOption{animals}{\gdef\@journal{animals}\gdef\@journalfull{Animals}\gdef\@journalshort{Animals}\gdef\@doiabbr{ani}\gdef\@ISSN{2076-2615}}
\DeclareOption{antibiotics}{\gdef\@journal{antibiotics}\gdef\@journalfull{Antibiotics}\gdef\@journalshort{Antibiotics}\gdef\@doiabbr{antibiotics}\gdef\@ISSN{2079-6382}}
\DeclareOption{antibodies}{\gdef\@journal{antibodies}\gdef\@journalfull{Antibodies}\gdef\@journalshort{Antibodies}\gdef\@doiabbr{antib}\gdef\@ISSN{2073-4468}}
\DeclareOption{antioxidants}{\gdef\@journal{antioxidants}\gdef\@journalfull{Antioxidants}\gdef\@journalshort{Antioxidants}\gdef\@doiabbr{antiox}\gdef\@ISSN{2076-3921}}
\DeclareOption{applbiosci}{\gdef\@journal{applbiosci}\gdef\@journalfull{Applied Biosciences}\gdef\@journalshort{Appl. Biosci.}\gdef\@doiabbr{applbiosci}\gdef\@ISSN{2813-0464}\gdef\@continuouspages{yes}}
\DeclareOption{appliedchem}{\gdef\@journal{appliedchem}\gdef\@journalfull{AppliedChem}\gdef\@journalshort{AppliedChem}\gdef\@doiabbr{appliedchem}\gdef\@ISSN{2673-9623}\gdef\@continuouspages{yes}}
\DeclareOption{appliedmath}{\gdef\@journal{appliedmath}\gdef\@journalfull{AppliedMath}\gdef\@journalshort{AppliedMath}\gdef\@doiabbr{appliedmath}\gdef\@ISSN{2673-9909}\gdef\@continuouspages{yes}}
\DeclareOption{applmech}{\gdef\@journal{applmech}\gdef\@journalfull{Applied Mechanics}\gdef\@journalshort{Appl. Mech.}\gdef\@doiabbr{applmech}\gdef\@ISSN{2673-3161}\gdef\@continuouspages{yes}}
\DeclareOption{applmicrobiol}{\gdef\@journal{applmicrobiol}\gdef\@journalfull{Applied Microbiology}\gdef\@journalshort{Appl. Microbiol.}\gdef\@doiabbr{applmicrobiol}\gdef\@ISSN{2673-8007}\gdef\@continuouspages{yes}}
\DeclareOption{applnano}{\gdef\@journal{applnano}\gdef\@journalfull{Applied Nano}\gdef\@journalshort{Appl. Nano}\gdef\@doiabbr{applnano}\gdef\@ISSN{2673-3501}\gdef\@continuouspages{yes}}
\DeclareOption{applsci}{\gdef\@journal{applsci}\gdef\@journalfull{Applied Sciences}\gdef\@journalshort{Appl. Sci.}\gdef\@doiabbr{app}\gdef\@ISSN{2076-3417}}
\DeclareOption{aquacj}{\gdef\@journal{aquacj}\gdef\@journalfull{Aquaculture Journal}\gdef\@journalshort{Aquac. J.}\gdef\@doiabbr{aj}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{architecture}{\gdef\@journal{architecture}\gdef\@journalfull{Architecture}\gdef\@journalshort{Architecture}\gdef\@doiabbr{architecture}\gdef\@ISSN{2673-8945}\gdef\@continuouspages{yes}}
\DeclareOption{arts}{\gdef\@journal{arts}\gdef\@journalfull{Arts}\gdef\@journalshort{Arts}\gdef\@doiabbr{arts}\gdef\@ISSN{2076-0752}}
\DeclareOption{asc}{\gdef\@journal{asc}\gdef\@journalfull{Automatic Systems and Control}\gdef\@journalshort{Autom. Syst. Control}\gdef\@doiabbr{}\gdef\@ISSN{}}
\DeclareOption{asi}{\gdef\@journal{asi}\gdef\@journalfull{Applied System Innovation}\gdef\@journalshort{Appl. Syst. Innov.}\gdef\@doiabbr{asi}\gdef\@ISSN{2571-5577}}
\DeclareOption{astronomy}{\gdef\@journal{astronomy}\gdef\@journalfull{Astronomy}\gdef\@journalshort{Astronomy}\gdef\@doiabbr{astronomy}\gdef\@ISSN{2674-0346}\gdef\@continuouspages{yes}}
\DeclareOption{atmosphere}{\gdef\@journal{atmosphere}\gdef\@journalfull{Atmosphere}\gdef\@journalshort{Atmosphere}\gdef\@doiabbr{atmos}\gdef\@ISSN{2073-4433}}
\DeclareOption{atoms}{\gdef\@journal{atoms}\gdef\@journalfull{Atoms}\gdef\@journalshort{Atoms}\gdef\@doiabbr{atoms}\gdef\@ISSN{2218-2004}}
\DeclareOption{audiolres}{\gdef\@journal{audiolres}\gdef\@journalfull{Audiology Research}\gdef\@journalshort{Audiol. Res.}\gdef\@doiabbr{audiolres}\gdef\@ISSN{2039-4349}\gdef\@continuouspages{yes}}
\DeclareOption{automation}{\gdef\@journal{automation}\gdef\@journalfull{Automation}\gdef\@journalshort{Automation}\gdef\@doiabbr{automation}\gdef\@ISSN{2673-4052}\gdef\@continuouspages{yes}}
\DeclareOption{axioms}{\gdef\@journal{axioms}\gdef\@journalfull{Axioms}\gdef\@journalshort{Axioms}\gdef\@doiabbr{axioms}\gdef\@ISSN{2075-1680}}
\DeclareOption{bacteria}{\gdef\@journal{bacteria}\gdef\@journalfull{Bacteria}\gdef\@journalshort{Bacteria}\gdef\@doiabbr{bacteria}\gdef\@ISSN{2674-1334}\gdef\@continuouspages{yes}}
\DeclareOption{batteries}{\gdef\@journal{batteries}\gdef\@journalfull{Batteries}\gdef\@journalshort{Batteries}\gdef\@doiabbr{batteries}\gdef\@ISSN{2313-0105}}
\DeclareOption{bdcc}{\gdef\@journal{bdcc}\gdef\@journalfull{Big Data and Cognitive Computing}\gdef\@journalshort{Big Data Cogn. Comput.}\gdef\@doiabbr{bdcc}\gdef\@ISSN{2504-2289}}
\DeclareOption{behavsci}{\gdef\@journal{behavsci}\gdef\@journalfull{Behavioral Sciences}\gdef\@journalshort{Behav. Sci.}\gdef\@doiabbr{bs}\gdef\@ISSN{2076-328X}}
\DeclareOption{beverages}{\gdef\@journal{beverages}\gdef\@journalfull{Beverages}\gdef\@journalshort{Beverages}\gdef\@doiabbr{beverages}\gdef\@ISSN{2306-5710}}
\DeclareOption{biochem}{\gdef\@journal{biochem}\gdef\@journalfull{BioChem}\gdef\@journalshort{BioChem}\gdef\@doiabbr{biochem}\gdef\@ISSN{2673-6411}\gdef\@continuouspages{yes}}
\DeclareOption{bioengineering}{\gdef\@journal{bioengineering}\gdef\@journalfull{Bioengineering}\gdef\@journalshort{Bioengineering}\gdef\@doiabbr{bioengineering}\gdef\@ISSN{2306-5354}}
\DeclareOption{biologics}{\gdef\@journal{biologics}\gdef\@journalfull{Biologics}\gdef\@journalshort{Biologics}\gdef\@doiabbr{biologics}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{biology}{\gdef\@journal{biology}\gdef\@journalfull{Biology}\gdef\@journalshort{Biology}\gdef\@doiabbr{biology}\gdef\@ISSN{2079-7737}}
\DeclareOption{biomass}{\gdef\@journal{biomass}\gdef\@journalfull{Biomass}\gdef\@journalshort{Biomass}\gdef\@doiabbr{biomass}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{biomechanics}{\gdef\@journal{biomechanics}\gdef\@journalfull{Biomechanics}\gdef\@journalshort{Biomechanics}\gdef\@doiabbr{biomechanics}\gdef\@ISSN{2673-7078}\gdef\@continuouspages{yes}}
\DeclareOption{biomed}{\gdef\@journal{biomed}\gdef\@journalfull{BioMed}\gdef\@journalshort{BioMed}\gdef\@doiabbr{biomed}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{biomedicines}{\gdef\@journal{biomedicines}\gdef\@journalfull{Biomedicines}\gdef\@journalshort{Biomedicines}\gdef\@doiabbr{biomedicines}\gdef\@ISSN{2227-9059}}
\DeclareOption{biomedinformatics}{\gdef\@journal{biomedinformatics}\gdef\@journalfull{Biomedinformatics}\gdef\@journalshort{Biomedinformatics}\gdef\@doiabbr{biomedinformatics}\gdef\@ISSN{2673-7426}\gdef\@continuouspages{yes}}
\DeclareOption{biomimetics}{\gdef\@journal{biomimetics}\gdef\@journalfull{Biomimetics}\gdef\@journalshort{Biomimetics}\gdef\@doiabbr{biomimetics}\gdef\@ISSN{2313-7673}}
\DeclareOption{biomolecules}{\gdef\@journal{biomolecules}\gdef\@journalfull{Biomolecules}\gdef\@journalshort{Biomolecules}\gdef\@doiabbr{biom}\gdef\@ISSN{2218-273X}}
\DeclareOption{biophysica}{\gdef\@journal{biophysica}\gdef\@journalfull{Biophysica}\gdef\@journalshort{Biophysica}\gdef\@doiabbr{biophysica}\gdef\@ISSN{2673-4125}\gdef\@continuouspages{yes}}
\DeclareOption{biosensors}{\gdef\@journal{biosensors}\gdef\@journalfull{Biosensors}\gdef\@journalshort{Biosensors}\gdef\@doiabbr{bios}\gdef\@ISSN{2079-6374}}
\DeclareOption{biotech}{\gdef\@journal{biotech}\gdef\@journalfull{BioTech}\gdef\@journalshort{BioTech}\gdef\@doiabbr{biotech}\gdef\@ISSN{2673-6284}}
\DeclareOption{birds}{\gdef\@journal{birds}\gdef\@journalfull{Birds}\gdef\@journalshort{Birds}\gdef\@doiabbr{birds}\gdef\@ISSN{2673-6004}\gdef\@continuouspages{yes}}
\DeclareOption{bloods}{\gdef\@journal{bloods}\gdef\@journalfull{Bloods}\gdef\@journalshort{Bloods}\gdef\@doiabbr{bloods}\gdef\@ISSN{2673-415X}}
\DeclareOption{blsf}{\gdef\@journal{blsf}\gdef\@journalfull{Biology and Life Sciences Forum}\gdef\@journalshort{Biol. Life Sci. Forum}\gdef\@doiabbr{blsf	}\gdef\@ISSN{2673-9976}}
\DeclareOption{brainsci}{\gdef\@journal{brainsci}\gdef\@journalfull{Brain Sciences}\gdef\@journalshort{Brain Sci.}\gdef\@doiabbr{brainsci}\gdef\@ISSN{2076-3425}}
\DeclareOption{breath}{\gdef\@journal{breath}\gdef\@journalfull{Breath}\gdef\@journalshort{Breath}\gdef\@doiabbr{breath}\gdef\@ISSN{}}
\DeclareOption{buildings}{\gdef\@journal{buildings}\gdef\@journalfull{Buildings}\gdef\@journalshort{Buildings}\gdef\@doiabbr{buildings}\gdef\@ISSN{2075-5309}}
\DeclareOption{businesses}{\gdef\@journal{businesses}\gdef\@journalfull{Businesses}\gdef\@journalshort{Businesses}\gdef\@doiabbr{businesses}\gdef\@ISSN{2673-7116}\gdef\@continuouspages{yes}}
\DeclareOption{cancers}{\gdef\@journal{cancers}\gdef\@journalfull{Cancers}\gdef\@journalshort{Cancers}\gdef\@doiabbr{cancers}\gdef\@ISSN{2072-6694}}
\DeclareOption{carbon}{\gdef\@journal{carbon}\gdef\@journalfull{C}\gdef\@journalshort{C}\gdef\@doiabbr{c}\gdef\@ISSN{2311-5629}}
\DeclareOption{cardiogenetics}{\gdef\@journal{cardiogenetics}\gdef\@journalfull{Cardiogenetics}\gdef\@journalshort{Cardiogenetics}\gdef\@doiabbr{cardiogenetics}\gdef\@ISSN{2035-8148}\gdef\@continuouspages{yes}}
\DeclareOption{catalysts}{\gdef\@journal{catalysts}\gdef\@journalfull{Catalysts}\gdef\@journalshort{Catalysts}\gdef\@doiabbr{catal}\gdef\@ISSN{2073-4344}}
\DeclareOption{cells}{\gdef\@journal{cells}\gdef\@journalfull{Cells}\gdef\@journalshort{Cells}\gdef\@doiabbr{cells}\gdef\@ISSN{2073-4409}}
\DeclareOption{ceramics}{\gdef\@journal{ceramics}\gdef\@journalfull{Ceramics}\gdef\@journalshort{Ceramics}\gdef\@doiabbr{ceramics}\gdef\@ISSN{2571-6131}\gdef\@continuouspages{yes}}
\DeclareOption{challenges}{\gdef\@journal{challenges}\gdef\@journalfull{Challenges}\gdef\@journalshort{Challenges}\gdef\@doiabbr{challe}\gdef\@ISSN{2078-1547}}
\DeclareOption{chemengineering}{\gdef\@journal{chemengineering}\gdef\@journalfull{ChemEngineering}\gdef\@journalshort{ChemEngineering}\gdef\@doiabbr{chemengineering}\gdef\@ISSN{2305-7084}}
\DeclareOption{chemistry}{\gdef\@journal{chemistry}\gdef\@journalfull{Chemistry}\gdef\@journalshort{Chemistry}\gdef\@doiabbr{chemistry}\gdef\@ISSN{2624-8549}\gdef\@continuouspages{yes}}
\DeclareOption{chemosensors}{\gdef\@journal{chemosensors}\gdef\@journalfull{Chemosensors}\gdef\@journalshort{Chemosensors}\gdef\@doiabbr{chemosensors}\gdef\@ISSN{2227-9040}}
\DeclareOption{chemproc}{\gdef\@journal{chemproc}\gdef\@journalfull{Chemistry Proceedings}\gdef\@journalshort{Chem. Proc.}\gdef\@doiabbr{chemproc}\gdef\@ISSN{2673-4583}}
\DeclareOption{children}{\gdef\@journal{children}\gdef\@journalfull{Children}\gdef\@journalshort{Children}\gdef\@doiabbr{children}\gdef\@ISSN{2227-9067}}
\DeclareOption{chips}{\gdef\@journal{chips}\gdef\@journalfull{Chips}\gdef\@journalshort{Chips}\gdef\@doiabbr{chips}\gdef\@ISSN{2674-0710}\gdef\@continuouspages{yes}}
\DeclareOption{cimb}{\gdef\@journal{cimb}\gdef\@journalfull{Current Issues in Molecular Biology}\gdef\@journalshort{Curr. Issues Mol. Biol.}\gdef\@doiabbr{cimb}\gdef\@ISSN{1467-3045}\gdef\@continuouspages{yes}}
\DeclareOption{civileng}{\gdef\@journal{civileng}\gdef\@journalfull{CivilEng}\gdef\@journalshort{CivilEng}\gdef\@doiabbr{civileng}\gdef\@ISSN{2673-4109}\gdef\@continuouspages{yes}}
\DeclareOption{cleantechnol}{\gdef\@journal{cleantechnol}\gdef\@journalfull{Clean Technologies}\gdef\@journalshort{Clean Technol.}\gdef\@doiabbr{cleantechnol}\gdef\@ISSN{2571-8797}\gdef\@continuouspages{yes}}
\DeclareOption{climate}{\gdef\@journal{climate}\gdef\@journalfull{Climate}\gdef\@journalshort{Climate}\gdef\@doiabbr{cli}\gdef\@ISSN{2225-1154}}
\DeclareOption{clinpract}{\gdef\@journal{clinpract}\gdef\@journalfull{Clinics and Practice}\gdef\@journalshort{Clin. Pract.}\gdef\@doiabbr{clinpract}\gdef\@ISSN{2039-7283}\gdef\@continuouspages{yes}}
\DeclareOption{clockssleep}{\gdef\@journal{clockssleep}\gdef\@journalfull{Clocks \& Sleep}\gdef\@journalshort{Clocks\&Sleep}\gdef\@doiabbr{clockssleep}\gdef\@ISSN{2624-5175}\gdef\@continuouspages{yes}}
\DeclareOption{cmd}{\gdef\@journal{cmd}\gdef\@journalfull{Corrosion and Materials Degradation}\gdef\@journalshort{Corros. Mater. Degrad.}\gdef\@doiabbr{cmd}\gdef\@ISSN{2624-5558}\gdef\@continuouspages{yes}}
\DeclareOption{coasts}{\gdef\@journal{coasts}\gdef\@journalfull{Coasts}\gdef\@journalshort{Coasts}\gdef\@doiabbr{coasts}\gdef\@ISSN{2673-964X}\gdef\@continuouspages{yes}}
\DeclareOption{coatings}{\gdef\@journal{coatings}\gdef\@journalfull{Coatings}\gdef\@journalshort{Coatings}\gdef\@doiabbr{coatings}\gdef\@ISSN{2079-6412}}
\DeclareOption{colloids}{\gdef\@journal{colloids}\gdef\@journalfull{Colloids Interfaces}\gdef\@journalshort{Colloids Interfaces}\gdef\@doiabbr{colloids}\gdef\@ISSN{2504-5377}}
\DeclareOption{colorants}{\gdef\@journal{colorants}\gdef\@journalfull{Colorants}\gdef\@journalshort{Colorants}\gdef\@doiabbr{colorants}\gdef\@ISSN{2079-6447}\gdef\@continuouspages{yes}}
\DeclareOption{commodities}{\gdef\@journal{commodities}\gdef\@journalfull{Commodities}\gdef\@journalshort{Commodities}\gdef\@doiabbr{commodities}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{compounds}{\gdef\@journal{compounds}\gdef\@journalfull{Compounds}\gdef\@journalshort{Compounds}\gdef\@doiabbr{compounds}\gdef\@ISSN{2673-6918}\gdef\@continuouspages{yes}}
\DeclareOption{computation}{\gdef\@journal{computation}\gdef\@journalfull{Computation}\gdef\@journalshort{Computation}\gdef\@doiabbr{computation}\gdef\@ISSN{2079-3197}}
\DeclareOption{computers}{\gdef\@journal{computers}\gdef\@journalfull{Computers}\gdef\@journalshort{Computers}\gdef\@doiabbr{computers}\gdef\@ISSN{2073-431X}}
\DeclareOption{condensedmatter}{\gdef\@journal{condensedmatter}\gdef\@journalfull{Condensed Matter}\gdef\@journalshort{Condens. Matter}\gdef\@doiabbr{condmat}\gdef\@ISSN{2410-3896}}
\DeclareOption{conservation}{\gdef\@journal{conservation}\gdef\@journalfull{Conservation}\gdef\@journalshort{Conservation}\gdef\@doiabbr{conservation}\gdef\@ISSN{2673-7159}\gdef\@continuouspages{yes}}
\DeclareOption{constrmater}{\gdef\@journal{constrmater}\gdef\@journalfull{Construction Materials}\gdef\@journalshort{Constr. Mater.}\gdef\@doiabbr{constrmater}\gdef\@ISSN{2673-7108}\gdef\@continuouspages{yes}}
\DeclareOption{cosmetics}{\gdef\@journal{cosmetics}\gdef\@journalfull{Cosmetics}\gdef\@journalshort{Cosmetics}\gdef\@doiabbr{cosmetics}\gdef\@ISSN{2079-9284}}
\DeclareOption{covid}{\gdef\@journal{covid}\gdef\@journalfull{COVID}\gdef\@journalshort{COVID}\gdef\@doiabbr{covid}\gdef\@ISSN{2673-8112}\gdef\@continuouspages{yes}}
\DeclareOption{crops}{\gdef\@journal{crops}\gdef\@journalfull{Crops}\gdef\@journalshort{Crops}\gdef\@doiabbr{crops}\gdef\@ISSN{2673-7655}\gdef\@continuouspages{yes}}
\DeclareOption{cryptography}{\gdef\@journal{cryptography}\gdef\@journalfull{Cryptography}\gdef\@journalshort{Cryptography}\gdef\@doiabbr{cryptography}\gdef\@ISSN{2410-387X}}
\DeclareOption{crystals}{\gdef\@journal{crystals}\gdef\@journalfull{Crystals}\gdef\@journalshort{Crystals}\gdef\@doiabbr{cryst}\gdef\@ISSN{2073-4352}}
\DeclareOption{csmf}{\gdef\@journal{csmf}\gdef\@journalfull{Computer Sciences \& Mathematics Forum}\gdef\@journalshort{Comput. Sci. Math. Forum}\gdef\@doiabbr{csmf}\gdef\@ISSN{2813-0324}\gdef\@continuouspages{yes}}
\DeclareOption{ctn}{\gdef\@journal{ctn}\gdef\@journalfull{Clinical and Translational Neuroscience}\gdef\@journalshort{CTN}\gdef\@doiabbr{Clin. Transl. Neurosci.}\gdef\@ISSN{2514-183X}}
\DeclareOption{curroncol}{\gdef\@journal{curroncol}\gdef\@journalfull{Current Oncology}\gdef\@journalshort{Curr. Oncol.}\gdef\@doiabbr{curroncol}\gdef\@ISSN{1718-7729}\gdef\@continuouspages{yes}}
\DeclareOption{cyber}{\gdef\@journal{cyber}\gdef\@journalfull{Cyber}\gdef\@journalshort{Cyber}\gdef\@doiabbr{cyber}\gdef\@ISSN{2624-800X}}
\DeclareOption{dairy}{\gdef\@journal{dairy}\gdef\@journalfull{Dairy}\gdef\@journalshort{Dairy}\gdef\@doiabbr{dairy}\gdef\@ISSN{2624-862X}\gdef\@continuouspages{yes}}
\DeclareOption{data}{\gdef\@journal{data}\gdef\@journalfull{Data}\gdef\@journalshort{Data}\gdef\@doiabbr{data}\gdef\@ISSN{2306-5729}}
\DeclareOption{dentistry}{\gdef\@journal{dentistry}\gdef\@journalfull{Dentistry Journal}\gdef\@journalshort{Dent. J.}\gdef\@doiabbr{dj}\gdef\@ISSN{2304-6767}}
\DeclareOption{dermato}{\gdef\@journal{dermato}\gdef\@journalfull{Dermato}\gdef\@journalshort{Dermato}\gdef\@doiabbr{dermato}\gdef\@ISSN{2673-6179}\gdef\@continuouspages{yes}}
\DeclareOption{dermatopathology}{\gdef\@journal{dermatopathology}\gdef\@journalfull{Dermatopathology}\gdef\@journalshort{Dermatopathology}\gdef\@doiabbr{dermatopathology}\gdef\@ISSN{2296-3529}\gdef\@continuouspages{yes}}
\DeclareOption{designs}{\gdef\@journal{designs}\gdef\@journalfull{Designs}\gdef\@journalshort{Designs}\gdef\@doiabbr{designs}\gdef\@ISSN{2411-9660}}
\DeclareOption{diabetology}{\gdef\@journal{diabetology}\gdef\@journalfull{Diabetology}\gdef\@journalshort{Diabetology}\gdef\@doiabbr{diabetology}\gdef\@ISSN{2673-4540}\gdef\@continuouspages{yes}}
\DeclareOption{diagnostics}{\gdef\@journal{diagnostics}\gdef\@journalfull{Diagnostics}\gdef\@journalshort{Diagnostics}\gdef\@doiabbr{diagnostics}\gdef\@ISSN{2075-4418}}
\DeclareOption{dietetics}{\gdef\@journal{dietetics}\gdef\@journalfull{Dietetics}\gdef\@journalshort{Dietetics}\gdef\@doiabbr{dietetics}\gdef\@ISSN{2674-0311}\gdef\@continuouspages{yes}}
\DeclareOption{digital}{\gdef\@journal{digital}\gdef\@journalfull{Digital}\gdef\@journalshort{Digital}\gdef\@doiabbr{digital}\gdef\@ISSN{2673-6470}\gdef\@continuouspages{yes}}
\DeclareOption{disabilities}{\gdef\@journal{disabilities}\gdef\@journalfull{Disabilities}\gdef\@journalshort{Disabilities}\gdef\@doiabbr{disabilities}\gdef\@ISSN{2673-7272}\gdef\@continuouspages{yes}}
\DeclareOption{diseases}{\gdef\@journal{diseases}\gdef\@journalfull{Diseases}\gdef\@journalshort{Diseases}\gdef\@doiabbr{diseases}\gdef\@ISSN{2079-9721}}
\DeclareOption{diversity}{\gdef\@journal{diversity}\gdef\@journalfull{Diversity}\gdef\@journalshort{Diversity}\gdef\@doiabbr{d}\gdef\@ISSN{1424-2818}}
\DeclareOption{dna}{\gdef\@journal{dna}\gdef\@journalfull{DNA}\gdef\@journalshort{DNA}\gdef\@doiabbr{dna}\gdef\@ISSN{2673-8856}\gdef\@continuouspages{yes}}
\DeclareOption{drones}{\gdef\@journal{drones}\gdef\@journalfull{Drones}\gdef\@journalshort{Drones}\gdef\@doiabbr{drones}\gdef\@ISSN{2504-446X}}
\DeclareOption{dynamics}{\gdef\@journal{dynamics}\gdef\@journalfull{Dynamics}\gdef\@journalshort{Dynamics}\gdef\@doiabbr{dynamics}\gdef\@ISSN{2673-8716}\gdef\@continuouspages{yes}}
\DeclareOption{earth}{\gdef\@journal{earth}\gdef\@journalfull{Earth}\gdef\@journalshort{Earth}\gdef\@doiabbr{earth}\gdef\@ISSN{2673-4834}\gdef\@continuouspages{yes}}
\DeclareOption{ebj}{\gdef\@journal{ebj}\gdef\@journalfull{European Burn Journal}\gdef\@journalshort{Eur. Burn J.}\gdef\@doiabbr{ebj}\gdef\@ISSN{2673-1991}\gdef\@continuouspages{yes}}
\DeclareOption{ecologies}{\gdef\@journal{ecologies}\gdef\@journalfull{Ecologies}\gdef\@journalshort{Ecologies}\gdef\@doiabbr{ecologies}\gdef\@ISSN{2673-4133}\gdef\@continuouspages{yes}}
\DeclareOption{econometrics}{\gdef\@journal{econometrics}\gdef\@journalfull{Econometrics}\gdef\@journalshort{Econometrics}\gdef\@doiabbr{econometrics}\gdef\@ISSN{2225-1146}}
\DeclareOption{economies}{\gdef\@journal{economies}\gdef\@journalfull{Economies}\gdef\@journalshort{Economies}\gdef\@doiabbr{economies}\gdef\@ISSN{2227-7099}}
\DeclareOption{education}{\gdef\@journal{education}\gdef\@journalfull{Education Sciences}\gdef\@journalshort{Educ. Sci.}\gdef\@doiabbr{educsci}\gdef\@ISSN{2227-7102}}
\DeclareOption{ejihpe}{\gdef\@journal{ejihpe}\gdef\@journalfull{European Journal of Investigation in Health Psychology and Education}\gdef\@journalshort{Eur. J. Investig. Health Psychol. Educ.}\gdef\@doiabbr{ejihpe}\gdef\@ISSN{2254-9625}\gdef\@continuouspages{yes}}
\DeclareOption{electricity}{\gdef\@journal{electricity}\gdef\@journalfull{Electricity}\gdef\@journalshort{Electricity}\gdef\@doiabbr{electricity}\gdef\@ISSN{2673-4826}\gdef\@continuouspages{yes}}
\DeclareOption{electrochem}{\gdef\@journal{electrochem}\gdef\@journalfull{Electrochem}\gdef\@journalshort{Electrochem}\gdef\@doiabbr{electrochem}\gdef\@ISSN{2673-3293}\gdef\@continuouspages{yes}}
\DeclareOption{electronicmat}{\gdef\@journal{electronicmat}\gdef\@journalfull{Electronic Materials}\gdef\@journalshort{Electron. Mater.}\gdef\@doiabbr{electronicmat}\gdef\@ISSN{2673-3978}\gdef\@continuouspages{yes}}
\DeclareOption{electronics}{\gdef\@journal{electronics}\gdef\@journalfull{Electronics}\gdef\@journalshort{Electronics}\gdef\@doiabbr{electronics}\gdef\@ISSN{2079-9292}}
\DeclareOption{encyclopedia}{\gdef\@journal{encyclopedia}\gdef\@journalfull{Encyclopedia}\gdef\@journalshort{Encyclopedia}\gdef\@doiabbr{encyclopedia}\gdef\@ISSN{2673-8392}\gdef\@continuouspages{yes}}
\DeclareOption{endocrines}{\gdef\@journal{endocrines}\gdef\@journalfull{Endocrines}\gdef\@journalshort{Endocrines}\gdef\@doiabbr{endocrines}\gdef\@ISSN{2673-396X}\gdef\@continuouspages{yes}}
\DeclareOption{energies}{\gdef\@journal{energies}\gdef\@journalfull{Energies}\gdef\@journalshort{Energies}\gdef\@doiabbr{en}\gdef\@ISSN{1996-1073}}
\DeclareOption{eng}{\gdef\@journal{eng}\gdef\@journalfull{Eng-Advances in Engineering}\gdef\@journalshort{Eng}\gdef\@doiabbr{eng}\gdef\@ISSN{2673-4117}\gdef\@continuouspages{yes}}
\DeclareOption{engproc}{\gdef\@journal{engproc}\gdef\@journalfull{Engineering Proceedings}\gdef\@journalshort{Eng. Proc.}\gdef\@doiabbr{engproc}\gdef\@ISSN{2673-4591}}
%\DeclareOption{ent}{\gdef\@journal{ent}\gdef\@journalfull{}\gdef\@journalshort{}\gdef\@doiabbr{}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{entomology}{\gdef\@journal{entomology}\gdef\@journalfull{Entomology}\gdef\@journalshort{Entomology}\gdef\@doiabbr{entomology}\gdef\@ISSN{2813-0502}\gdef\@continuouspages{yes}}	
\DeclareOption{entropy}{\gdef\@journal{entropy}\gdef\@journalfull{Entropy}\gdef\@journalshort{Entropy}\gdef\@doiabbr{e}\gdef\@ISSN{1099-4300}}
\DeclareOption{environments}{\gdef\@journal{environments}\gdef\@journalfull{Environments}\gdef\@journalshort{Environments}\gdef\@doiabbr{environments}\gdef\@ISSN{2076-3298}}
\DeclareOption{environsciproc}{\gdef\@journal{environsciproc}\gdef\@journalfull{Environmental Sciences Proceedings}\gdef\@journalshort{Environ. Sci. Proc.}\gdef\@doiabbr{environsciproc}\gdef\@ISSN{2673-4931}}
\DeclareOption{epidemiologia}{\gdef\@journal{epidemiologia}\gdef\@journalfull{Epidemiologia}\gdef\@journalshort{Epidemiologia}\gdef\@doiabbr{epidemiologia}\gdef\@ISSN{2673-3986}\gdef\@continuouspages{yes}}
\DeclareOption{epigenomes}{\gdef\@journal{epigenomes}\gdef\@journalfull{Epigenomes}\gdef\@journalshort{Epigenomes}\gdef\@doiabbr{epigenomes}\gdef\@ISSN{2075-4655}}
\DeclareOption{est}{\gdef\@journal{est}\gdef\@journalfull{Electrochemical Science and Technology}\gdef\@journalshort{Electrochem. Sci. Technol.}\gdef\@doiabbr{}\gdef\@ISSN{}}
\DeclareOption{fermentation}{\gdef\@journal{fermentation}\gdef\@journalfull{Fermentation}\gdef\@journalshort{Fermentation}\gdef\@doiabbr{fermentation}\gdef\@ISSN{2311-5637}}
\DeclareOption{fibers}{\gdef\@journal{fibers}\gdef\@journalfull{Fibers}\gdef\@journalshort{Fibers}\gdef\@doiabbr{fib}\gdef\@ISSN{2079-6439}}
\DeclareOption{fintech}{\gdef\@journal{fintech}\gdef\@journalfull{FinTech}\gdef\@journalshort{FinTech}\gdef\@doiabbr{fintech}\gdef\@ISSN{2674-1032}\gdef\@continuouspages{yes}}
\DeclareOption{fire}{\gdef\@journal{fire}\gdef\@journalfull{Fire}\gdef\@journalshort{Fire}\gdef\@doiabbr{fire}\gdef\@ISSN{2571-6255}}
\DeclareOption{fishes}{\gdef\@journal{fishes}\gdef\@journalfull{Fishes}\gdef\@journalshort{Fishes}\gdef\@doiabbr{fishes}\gdef\@ISSN{2410-3888}}
\DeclareOption{fluids}{\gdef\@journal{fluids}\gdef\@journalfull{Fluids}\gdef\@journalshort{Fluids}\gdef\@doiabbr{fluids}\gdef\@ISSN{2311-5521}}
\DeclareOption{foods}{\gdef\@journal{foods}\gdef\@journalfull{Foods}\gdef\@journalshort{Foods}\gdef\@doiabbr{foods}\gdef\@ISSN{2304-8158}}
\DeclareOption{forecasting}{\gdef\@journal{forecasting}\gdef\@journalfull{Forecasting}\gdef\@journalshort{Forecasting}\gdef\@doiabbr{forecast}\gdef\@ISSN{2571-9394}\gdef\@continuouspages{yes}}
\DeclareOption{forensicsci}{\gdef\@journal{forensicsci}\gdef\@journalfull{Forensic Sciences}\gdef\@journalshort{Forensic Sci.}\gdef\@doiabbr{forensicsci}\gdef\@ISSN{2673-6756}\gdef\@continuouspages{yes}}
\DeclareOption{forests}{\gdef\@journal{forests}\gdef\@journalfull{Forests}\gdef\@journalshort{Forests}\gdef\@doiabbr{f}\gdef\@ISSN{1999-4907}}
\DeclareOption{foundations}{\gdef\@journal{foundations}\gdef\@journalfull{Foundations}\gdef\@journalshort{Foundations}\gdef\@doiabbr{foundations}\gdef\@ISSN{2673-9321}\gdef\@continuouspages{yes}}
\DeclareOption{fractalfract}{\gdef\@journal{fractalfract}\gdef\@journalfull{Fractal and Fractional}\gdef\@journalshort{Fractal Fract.}\gdef\@doiabbr{fractalfract}\gdef\@ISSN{2504-3110}}
\DeclareOption{fuels}{\gdef\@journal{fuels}\gdef\@journalfull{Fuels}\gdef\@journalshort{Fuels}\gdef\@doiabbr{fuels}\gdef\@ISSN{2673-3994}\gdef\@continuouspages{yes}}
\DeclareOption{futureinternet}{\gdef\@journal{futureinternet}\gdef\@journalfull{Future Internet}\gdef\@journalshort{Future Internet}\gdef\@doiabbr{fi}\gdef\@ISSN{1999-5903}}
%\DeclareOption{futureparasites}{\gdef\@journal{futureparasites}\gdef\@journalfull{}\gdef\@journalshort{}\gdef\@doiabbr{}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{futurepharmacol}{\gdef\@journal{futurepharmacol}\gdef\@journalfull{Future Pharmacology}\gdef\@journalshort{Future Pharm.}\gdef\@doiabbr{futurepharmacol}\gdef\@ISSN{2673-9879}\gdef\@continuouspages{yes}}
\DeclareOption{futurephys}{\gdef\@journal{futurephys}\gdef\@journalfull{Future Physics}\gdef\@journalshort{Future Phys.}\gdef\@doiabbr{futurephys}\gdef\@ISSN{2624-6503}}
\DeclareOption{futuretransp}{\gdef\@journal{futuretransp}\gdef\@journalfull{Future Transportation}\gdef\@journalshort{Future Transp.}\gdef\@doiabbr{futuretransp}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{galaxies}{\gdef\@journal{galaxies}\gdef\@journalfull{Galaxies}\gdef\@journalshort{Galaxies}\gdef\@doiabbr{galaxies}\gdef\@ISSN{2075-4434}}
\DeclareOption{games}{\gdef\@journal{games}\gdef\@journalfull{Games}\gdef\@journalshort{Games}\gdef\@doiabbr{g}\gdef\@ISSN{2073-4336}}
\DeclareOption{gases}{\gdef\@journal{gases}\gdef\@journalfull{Gases}\gdef\@journalshort{Gases}\gdef\@doiabbr{gases}\gdef\@ISSN{2673-5628}\gdef\@continuouspages{yes}}
\DeclareOption{gastroent}{\gdef\@journal{gastroent}\gdef\@journalfull{Gastroenterology Insights}\gdef\@journalshort{Gastroenterol. Insights}\gdef\@doiabbr{gastroent}\gdef\@ISSN{2036-7422}\gdef\@continuouspages{yes}}
\DeclareOption{gastrointestdisord}{\gdef\@journal{gastrointestdisord}\gdef\@journalfull{Gastrointestinal Disorders}\gdef\@journalshort{Gastrointest. Disord.}\gdef\@doiabbr{gidisord}\gdef\@ISSN{2624-5647}\gdef\@continuouspages{yes}}
\DeclareOption{gels}{\gdef\@journal{gels}\gdef\@journalfull{Gels}\gdef\@journalshort{Gels}\gdef\@doiabbr{gels}\gdef\@ISSN{2310-2861}}
\DeclareOption{genealogy}{\gdef\@journal{genealogy}\gdef\@journalfull{Genealogy}\gdef\@journalshort{Genealogy}\gdef\@doiabbr{genealogy}\gdef\@ISSN{2313-5778}}
\DeclareOption{genes}{\gdef\@journal{genes}\gdef\@journalfull{Genes}\gdef\@journalshort{Genes}\gdef\@doiabbr{genes}\gdef\@ISSN{2073-4425}}
\DeclareOption{geographies}{\gdef\@journal{geographies}\gdef\@journalfull{Geographies}\gdef\@journalshort{Geographies}\gdef\@doiabbr{geographies}\gdef\@ISSN{2673-7086}\gdef\@continuouspages{yes}}
\DeclareOption{geohazards}{\gdef\@journal{geohazards}\gdef\@journalfull{GeoHazards}\gdef\@journalshort{GeoHazards}\gdef\@doiabbr{geohazards}\gdef\@ISSN{2624-795X}\gdef\@continuouspages{yes}}
\DeclareOption{geomatics}{\gdef\@journal{geomatics}\gdef\@journalfull{Geomatics}\gdef\@journalshort{Geomatics}\gdef\@doiabbr{geomatics}\gdef\@ISSN{2673-7418}\gdef\@continuouspages{yes}}
\DeclareOption{geosciences}{\gdef\@journal{geosciences}\gdef\@journalfull{Geosciences}\gdef\@journalshort{Geosciences}\gdef\@doiabbr{geosciences}\gdef\@ISSN{2076-3263}}
\DeclareOption{geotechnics}{\gdef\@journal{geotechnics}\gdef\@journalfull{Geotechnics}\gdef\@journalshort{Geotechnics}\gdef\@doiabbr{geotechnics}\gdef\@ISSN{2673-7094}\gdef\@continuouspages{yes}}
\DeclareOption{geriatrics}{\gdef\@journal{geriatrics}\gdef\@journalfull{Geriatrics}\gdef\@journalshort{Geriatrics}\gdef\@doiabbr{geriatrics}\gdef\@ISSN{2308-3417}}
\DeclareOption{grasses}{\gdef\@journal{grasses}\gdef\@journalfull{Grasses}\gdef\@journalshort{Grasses}\gdef\@doiabbr{grasses}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{hazardousmatters}{\gdef\@journal{hazardousmatters}\gdef\@journalfull{Hazardous Matters}\gdef\@journalshort{Hazard. Matters}\gdef\@doiabbr{}\gdef\@ISSN{0014-0014}}
\DeclareOption{healthcare}{\gdef\@journal{healthcare}\gdef\@journalfull{Healthcare}\gdef\@journalshort{Healthcare}\gdef\@doiabbr{healthcare}\gdef\@ISSN{2227-9032}}
\DeclareOption{hearts}{\gdef\@journal{hearts}\gdef\@journalfull{Hearts}\gdef\@journalshort{Hearts}\gdef\@doiabbr{hearts}\gdef\@ISSN{2673-3846}\gdef\@continuouspages{yes}}
\DeclareOption{hemato}{\gdef\@journal{hemato}\gdef\@journalfull{Hemato}\gdef\@journalshort{Hemato}\gdef\@doiabbr{hemato}\gdef\@ISSN{2673-6357}\gdef\@continuouspages{yes}}
\DeclareOption{heritage}{\gdef\@journal{heritage}\gdef\@journalfull{Heritage}\gdef\@journalshort{Heritage}\gdef\@doiabbr{heritage}\gdef\@ISSN{2571-9408}\gdef\@continuouspages{yes}}
\DeclareOption{highthroughput}{\gdef\@journal{highthroughput}\gdef\@journalfull{High-Throughput}\gdef\@journalshort{High-Throughput}\gdef\@doiabbr{ht}\gdef\@ISSN{2571-5135}}
\DeclareOption{histories}{\gdef\@journal{histories}\gdef\@journalfull{Histories}\gdef\@journalshort{Histories}\gdef\@doiabbr{histories}\gdef\@ISSN{2409-9252}\gdef\@continuouspages{yes}}
\DeclareOption{horticulturae}{\gdef\@journal{horticulturae}\gdef\@journalfull{Horticulturae}\gdef\@journalshort{Horticulturae}\gdef\@doiabbr{horticulturae}\gdef\@ISSN{2311-7524}}
\DeclareOption{humanities}{\gdef\@journal{humanities}\gdef\@journalfull{Humanities}\gdef\@journalshort{Humanities}\gdef\@doiabbr{h}\gdef\@ISSN{2076-0787}}
\DeclareOption{humans}{\gdef\@journal{humans}\gdef\@journalfull{Humans}\gdef\@journalshort{Humans}\gdef\@doiabbr{humans}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{hydrobiology}{\gdef\@journal{hydrobiology}\gdef\@journalfull{Hydrobiology}\gdef\@journalshort{Hydrobiology	}\gdef\@doiabbr{hydrobiology}\gdef\@ISSN{2673-9917}\gdef\@continuouspages{yes}}
\DeclareOption{hydrogen}{\gdef\@journal{hydrogen}\gdef\@journalfull{Hydrogen}\gdef\@journalshort{Hydrogen}\gdef\@doiabbr{hydrogen}\gdef\@ISSN{2673-4141}\gdef\@continuouspages{yes}}
\DeclareOption{hydrology}{\gdef\@journal{hydrology}\gdef\@journalfull{Hydrology}\gdef\@journalshort{Hydrology}\gdef\@doiabbr{hydrology}\gdef\@ISSN{2306-5338}}
\DeclareOption{hygiene}{\gdef\@journal{hygiene}\gdef\@journalfull{Hygiene}\gdef\@journalshort{Hygiene}\gdef\@doiabbr{hygiene}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{idr}{\gdef\@journal{idr}\gdef\@journalfull{Infectious Disease Reports}\gdef\@journalshort{Infect. Dis. Rep.}\gdef\@doiabbr{idr}\gdef\@ISSN{2036-7449}\gdef\@continuouspages{yes}}
\DeclareOption{ijerph}{\gdef\@journal{ijerph}\gdef\@journalfull{International Journal of Environmental Research and Public Health}\gdef\@journalshort{Int. J. Environ. Res. Public Health}\gdef\@doiabbr{ijerph}\gdef\@ISSN{1660-4601}}
\DeclareOption{ijfs}{\gdef\@journal{ijfs}\gdef\@journalfull{International Journal of Financial Studies}\gdef\@journalshort{Int. J. Financial Stud.}\gdef\@doiabbr{ijfs}\gdef\@ISSN{2227-7072}}
\DeclareOption{ijgi}{\gdef\@journal{ijgi}\gdef\@journalfull{ISPRS International Journal of Geo-Information}\gdef\@journalshort{ISPRS Int. J. Geo-Inf.}\gdef\@doiabbr{ijgi}\gdef\@ISSN{2220-9964}}
\DeclareOption{ijms}{\gdef\@journal{ijms}\gdef\@journalfull{International Journal of Molecular Sciences}\gdef\@journalshort{Int. J. Mol. Sci.}\gdef\@doiabbr{ijms}\gdef\@ISSN{1422-0067}}
\DeclareOption{ijns}{\gdef\@journal{ijns}\gdef\@journalfull{International Journal of Neonatal Screening}\gdef\@journalshort{Int. J. Neonatal Screen.}\gdef\@doiabbr{ijns}\gdef\@ISSN{2409-515X}}
\DeclareOption{ijtm}{\gdef\@journal{ijtm}\gdef\@journalfull{International Journal of Translational Medicine}\gdef\@journalshort{Int. J. Transl. Med.}\gdef\@doiabbr{ijtm}\gdef\@ISSN{2673-8937}\gdef\@continuouspages{yes}}
\DeclareOption{ijtpp}{\gdef\@journal{ijtpp}\gdef\@journalfull{International Journal of Turbomachinery Propulsion and Power}\gdef\@journalshort{Int. J. Turbomach. Propuls. Power}\gdef\@doiabbr{ijtpp}\gdef\@ISSN{2504-186X}}
\DeclareOption{immuno}{\gdef\@journal{immuno}\gdef\@journalfull{Immuno}\gdef\@journalshort{Immuno}\gdef\@doiabbr{immuno}\gdef\@ISSN{2673-5601}\gdef\@continuouspages{yes}}
\DeclareOption{informatics}{\gdef\@journal{informatics}\gdef\@journalfull{Informatics}\gdef\@journalshort{Informatics}\gdef\@doiabbr{informatics}\gdef\@ISSN{2227-9709}}
\DeclareOption{information}{\gdef\@journal{information}\gdef\@journalfull{Information}\gdef\@journalshort{Information}\gdef\@doiabbr{info}\gdef\@ISSN{2078-2489}}
\DeclareOption{infrastructures}{\gdef\@journal{infrastructures}\gdef\@journalfull{Infrastructures}\gdef\@journalshort{Infrastructures}\gdef\@doiabbr{infrastructures}\gdef\@ISSN{2412-3811}}
\DeclareOption{inorganics}{\gdef\@journal{inorganics}\gdef\@journalfull{Inorganics}\gdef\@journalshort{Inorganics}\gdef\@doiabbr{inorganics}\gdef\@ISSN{2304-6740}}
\DeclareOption{insects}{\gdef\@journal{insects}\gdef\@journalfull{Insects}\gdef\@journalshort{Insects}\gdef\@doiabbr{insects}\gdef\@ISSN{2075-4450}}
\DeclareOption{instruments}{\gdef\@journal{instruments}\gdef\@journalfull{Instruments}\gdef\@journalshort{Instruments}\gdef\@doiabbr{instruments}\gdef\@ISSN{2410-390X}}
\DeclareOption{inventions}{\gdef\@journal{inventions}\gdef\@journalfull{Inventions}\gdef\@journalshort{Inventions}\gdef\@doiabbr{inventions}\gdef\@ISSN{2411-5134}}
\DeclareOption{iot}{\gdef\@journal{iot}\gdef\@journalfull{IoT}\gdef\@journalshort{IoT}\gdef\@doiabbr{iot}\gdef\@ISSN{2624-831X}\gdef\@continuouspages{yes}}
\DeclareOption{j}{\gdef\@journal{j}\gdef\@journalfull{J}\gdef\@journalshort{J}\gdef\@doiabbr{j}\gdef\@ISSN{2571-8800}\gdef\@continuouspages{yes}}
\DeclareOption{jal}{\gdef\@journal{jal}\gdef\@journalfull{Journal of Ageing and Longevity}\gdef\@journalshort{J. Ageing Longev.}\gdef\@doiabbr{jal}\gdef\@ISSN{2673-9259}\gdef\@continuouspages{yes}}
\DeclareOption{jcdd}{\gdef\@journal{jcdd}\gdef\@journalfull{Journal of Cardiovascular Development and Disease}\gdef\@journalshort{J. Cardiovasc. Dev. Dis.}\gdef\@doiabbr{jcdd}\gdef\@ISSN{2308-3425}}
\DeclareOption{jcm}{\gdef\@journal{jcm}\gdef\@journalfull{Journal of Clinical Medicine}\gdef\@journalshort{J. Clin. Med.}\gdef\@doiabbr{jcm}\gdef\@ISSN{2077-0383}}
\DeclareOption{jcp}{\gdef\@journal{jcp}\gdef\@journalfull{Journal of Cybersecurity and Privacy}\gdef\@journalshort{J. Cybersecur. Priv.}\gdef\@doiabbr{jcp}\gdef\@ISSN{2624-800X}\gdef\@continuouspages{yes}}
\DeclareOption{jcs}{\gdef\@journal{jcs}\gdef\@journalfull{Journal of Composites Science}\gdef\@journalshort{J. Compos. Sci.}\gdef\@doiabbr{jcs}\gdef\@ISSN{2504-477X}}
\DeclareOption{jcto}{\gdef\@journal{jcto}\gdef\@journalfull{Journal of Clinical \& Translational Ophthalmology}\gdef\@journalshort{J. Clin. Transl. Ophthalmol.}\gdef\@doiabbr{jcto}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{jdb}{\gdef\@journal{jdb}\gdef\@journalfull{Journal of Developmental Biology}\gdef\@journalshort{J. Dev. Biol.}\gdef\@doiabbr{jdb}\gdef\@ISSN{2221-3759}}
\DeclareOption{jeta}{\gdef\@journal{jeta}\gdef\@journalfull{Journal of Experimental and Theoretical Analyses}\gdef\@journalshort{J. Exp. Theor. Anal.}\gdef\@doiabbr{jeta}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{jfb}{\gdef\@journal{jfb}\gdef\@journalfull{Journal of Functional Biomaterials}\gdef\@journalshort{J. Funct. Biomater.}\gdef\@doiabbr{jfb}\gdef\@ISSN{2079-4983}}
\DeclareOption{jfmk}{\gdef\@journal{jfmk}\gdef\@journalfull{Journal of Functional Morphology and Kinesiology}\gdef\@journalshort{J. Funct. Morphol. Kinesiol.}\gdef\@doiabbr{jfmk}\gdef\@ISSN{2411-5142}}
\DeclareOption{jimaging}{\gdef\@journal{jimaging}\gdef\@journalfull{Journal of Imaging}\gdef\@journalshort{J. Imaging}\gdef\@doiabbr{jimaging}\gdef\@ISSN{2313-433X}}
\DeclareOption{jintelligence}{\gdef\@journal{jintelligence}\gdef\@journalfull{Journal of Intelligence}\gdef\@journalshort{J. Intell.}\gdef\@doiabbr{jintelligence}\gdef\@ISSN{2079-3200}}
\DeclareOption{jlpea}{\gdef\@journal{jlpea}\gdef\@journalfull{Journal of Low Power Electronics and Applications}\gdef\@journalshort{J. Low Power Electron. Appl.}\gdef\@doiabbr{jlpea}\gdef\@ISSN{2079-9268}}
\DeclareOption{jmmp}{\gdef\@journal{jmmp}\gdef\@journalfull{Journal of Manufacturing and Materials Processing}\gdef\@journalshort{J. Manuf. Mater. Process.}\gdef\@doiabbr{jmmp}\gdef\@ISSN{2504-4494}}
\DeclareOption{jmp}{\gdef\@journal{jmp}\gdef\@journalfull{Journal of Molecular Pathology}\gdef\@journalshort{J. Mol. Pathol.}\gdef\@doiabbr{jmp}\gdef\@ISSN{2673-5261}\gdef\@continuouspages{yes}}
\DeclareOption{jmse}{\gdef\@journal{jmse}\gdef\@journalfull{Journal of Marine Science and Engineering}\gdef\@journalshort{J. Mar. Sci. Eng.}\gdef\@doiabbr{jmse}\gdef\@ISSN{2077-1312}}
\DeclareOption{jne}{\gdef\@journal{jne}\gdef\@journalfull{Journal of Nuclear Engineering}\gdef\@journalshort{J. Nucl. Eng.}\gdef\@doiabbr{jne}\gdef\@ISSN{2673-4362}\gdef\@continuouspages{yes}}
\DeclareOption{jnt}{\gdef\@journal{jnt}\gdef\@journalfull{Journal of Nanotheranostics}\gdef\@journalshort{J. Nanotheranostics}\gdef\@doiabbr{jnt}\gdef\@ISSN{2624-845X}\gdef\@continuouspages{yes}}
\DeclareOption{jof}{\gdef\@journal{jof}\gdef\@journalfull{Journal of Fungi}\gdef\@journalshort{J. Fungi}\gdef\@doiabbr{jof}\gdef\@ISSN{2309-608X}}
\DeclareOption{joitmc}{\gdef\@journal{joitmc}\gdef\@journalfull{Journal of Open Innovation: Technology Market and Complexity}\gdef\@journalshort{J. Open Innov. Technol. Mark. Complex.}\gdef\@doiabbr{joitmc}\gdef\@ISSN{2199-8531}}
\DeclareOption{jor}{\gdef\@journal{jor}\gdef\@journalfull{Journal of Respiration}\gdef\@journalshort{J. Respir.}\gdef\@doiabbr{jor}\gdef\@ISSN{2673-527X}\gdef\@continuouspages{yes}}
\DeclareOption{journalmedia}{\gdef\@journal{journalmedia}\gdef\@journalfull{Journalism and Media}\gdef\@journalshort{Journal. Media}\gdef\@doiabbr{journalmedia}\gdef\@ISSN{2673-5172}\gdef\@continuouspages{yes}}
\DeclareOption{jox}{\gdef\@journal{jox}\gdef\@journalfull{Journal of Xenobiotics}\gdef\@journalshort{J. Xenobiot.}\gdef\@doiabbr{jox}\gdef\@ISSN{2039-4713}\gdef\@continuouspages{yes}}
\DeclareOption{jpm}{\gdef\@journal{jpm}\gdef\@journalfull{Journal of Personalized Medicine}\gdef\@journalshort{J. Pers. Med.}\gdef\@doiabbr{jpm}\gdef\@ISSN{2075-4426}}
\DeclareOption{jrfm}{\gdef\@journal{jrfm}\gdef\@journalfull{Journal of Risk and Financial Management}\gdef\@journalshort{J. Risk Financial Manag.}\gdef\@doiabbr{jrfm}\gdef\@ISSN{1911-8074}}
\DeclareOption{jsan}{\gdef\@journal{jsan}\gdef\@journalfull{Journal of Sensor and Actuator Networks}\gdef\@journalshort{J. Sens. Actuator Netw.}\gdef\@doiabbr{jsan}\gdef\@ISSN{2224-2708}}
\DeclareOption{jtaer}{\gdef\@journal{jtaer}\gdef\@journalfull{Journal of Theoretical and Applied Electronic Commerce Research}\gdef\@journalshort{J. Theor. Appl. Electron. Commer. Res.}\gdef\@doiabbr{jtaer}\gdef\@ISSN{0718-1876}\gdef\@continuouspages{yes}}
\DeclareOption{jzbg}{\gdef\@journal{jzbg}\gdef\@journalfull{Journal of Zoological and Botanical Gardens}\gdef\@journalshort{J. Zool. Bot. Gard.}\gdef\@doiabbr{jzbg}\gdef\@ISSN{2673-5636}\gdef\@continuouspages{yes}}
%\DeclareOption{kidney}{\gdef\@journal{kidney}\gdef\@journalfull{}\gdef\@journalshort{}\gdef\@doiabbr{}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{kidneydial}{\gdef\@journal{kidneydial}\gdef\@journalfull{Kidney and Dialysis}\gdef\@journalshort{Kidney Dial.}\gdef\@doiabbr{kidneydial}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{knowledge}{\gdef\@journal{knowledge}\gdef\@journalfull{Knowledge}\gdef\@journalshort{Knowledge}\gdef\@doiabbr{knowledge}\gdef\@ISSN{2673-9585}\gdef\@continuouspages{yes}}
\DeclareOption{land}{\gdef\@journal{land}\gdef\@journalfull{Land}\gdef\@journalshort{Land}\gdef\@doiabbr{land}\gdef\@ISSN{2073-445X}}
\DeclareOption{languages}{\gdef\@journal{languages}\gdef\@journalfull{Languages}\gdef\@journalshort{Languages}\gdef\@doiabbr{languages}\gdef\@ISSN{2226-471X}}
\DeclareOption{laws}{\gdef\@journal{laws}\gdef\@journalfull{Laws}\gdef\@journalshort{Laws}\gdef\@doiabbr{laws}\gdef\@ISSN{2075-471X}}
\DeclareOption{life}{\gdef\@journal{life}\gdef\@journalfull{Life}\gdef\@journalshort{Life}\gdef\@doiabbr{life}\gdef\@ISSN{2075-1729}}
\DeclareOption{liquids}{\gdef\@journal{liquids}\gdef\@journalfull{Liquids}\gdef\@journalshort{Liquids}\gdef\@doiabbr{liquids}\gdef\@ISSN{2673-8015}\gdef\@continuouspages{yes}}
\DeclareOption{literature}{\gdef\@journal{literature}\gdef\@journalfull{Literature}\gdef\@journalshort{Literature}\gdef\@doiabbr{literature}\gdef\@ISSN{2410-9789}\gdef\@continuouspages{yes}}
\DeclareOption{livers}{\gdef\@journal{livers}\gdef\@journalfull{Livers}\gdef\@journalshort{Livers}\gdef\@doiabbr{livers}\gdef\@ISSN{2673-4389}\gdef\@continuouspages{yes}}
\DeclareOption{logics}{\gdef\@journal{logics}\gdef\@journalfull{Logics}\gdef\@journalshort{Logics}\gdef\@doiabbr{logics}\gdef\@ISSN{2813-0405}\gdef\@continuouspages{yes}}
\DeclareOption{logistics}{\gdef\@journal{logistics}\gdef\@journalfull{Logistics}\gdef\@journalshort{Logistics}\gdef\@doiabbr{logistics}\gdef\@ISSN{2305-6290}}
\DeclareOption{lubricants}{\gdef\@journal{lubricants}\gdef\@journalfull{Lubricants}\gdef\@journalshort{Lubricants}\gdef\@doiabbr{lubricants}\gdef\@ISSN{2075-4442}}
\DeclareOption{lymphatics}{\gdef\@journal{lymphatics}\gdef\@journalfull{Lymphatics}\gdef\@journalshort{Lymphatics}\gdef\@doiabbr{lymphatics}\gdef\@ISSN{}\gdef\@continuouspages{yes}}	
\DeclareOption{machines}{\gdef\@journal{machines}\gdef\@journalfull{Machines}\gdef\@journalshort{Machines}\gdef\@doiabbr{machines}\gdef\@ISSN{2075-1702}}
\DeclareOption{macromol}{\gdef\@journal{macromol}\gdef\@journalfull{Macromol}\gdef\@journalshort{Macromol}\gdef\@doiabbr{macromol}\gdef\@ISSN{2673-6209}\gdef\@continuouspages{yes}}
\DeclareOption{magnetism}{\gdef\@journal{magnetism}\gdef\@journalfull{Magnetism}\gdef\@journalshort{Magnetism}\gdef\@doiabbr{magnetism}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{magnetochemistry}{\gdef\@journal{magnetochemistry}\gdef\@journalfull{Magnetochemistry}\gdef\@journalshort{Magnetochemistry}\gdef\@doiabbr{magnetochemistry}\gdef\@ISSN{2312-7481}}
\DeclareOption{make}{\gdef\@journal{make}\gdef\@journalfull{Machine Learning and Knowledge Extraction}\gdef\@journalshort{Mach. Learn. Knowl. Extr.}\gdef\@doiabbr{make}\gdef\@ISSN{2504-4990}\gdef\@continuouspages{yes}}
\DeclareOption{marinedrugs}{\gdef\@journal{marinedrugs}\gdef\@journalfull{Marine Drugs}\gdef\@journalshort{Mar. Drugs}\gdef\@doiabbr{md}\gdef\@ISSN{1660-3397}}
\DeclareOption{materials}{\gdef\@journal{materials}\gdef\@journalfull{Materials}\gdef\@journalshort{Materials}\gdef\@doiabbr{ma}\gdef\@ISSN{1996-1944}}
\DeclareOption{materproc}{\gdef\@journal{materproc}\gdef\@journalfull{Materials Proceedings}\gdef\@journalshort{Mater. Proc.}\gdef\@doiabbr{materproc}\gdef\@ISSN{2673-4605}}
\DeclareOption{mathematics}{\gdef\@journal{mathematics}\gdef\@journalfull{Mathematics}\gdef\@journalshort{Mathematics}\gdef\@doiabbr{math}\gdef\@ISSN{2227-7390}}
\DeclareOption{mca}{\gdef\@journal{mca}\gdef\@journalfull{Mathematical and Computational Applications}\gdef\@journalshort{Math. Comput. Appl.}\gdef\@doiabbr{mca}\gdef\@ISSN{2297-8747}}
\DeclareOption{measurements}{\gdef\@journal{measurements}\gdef\@journalfull{Measurements}\gdef\@journalshort{Measurements}\gdef\@doiabbr{measurements}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{medicina}{\gdef\@journal{medicina}\gdef\@journalfull{Medicina}\gdef\@journalshort{Medicina}\gdef\@doiabbr{medicina}\gdef\@ISSN{1648-9144}}
\DeclareOption{medicines}{\gdef\@journal{medicines}\gdef\@journalfull{Medicines}\gdef\@journalshort{Medicines}\gdef\@doiabbr{medicines}\gdef\@ISSN{2305-6320}}
\DeclareOption{medsci}{\gdef\@journal{medsci}\gdef\@journalfull{Medical Sciences}\gdef\@journalshort{Med. Sci.}\gdef\@doiabbr{medsci}\gdef\@ISSN{2076-3271}}
\DeclareOption{membranes}{\gdef\@journal{membranes}\gdef\@journalfull{Membranes}\gdef\@journalshort{Membranes}\gdef\@doiabbr{membranes}\gdef\@ISSN{2077-0375}}
\DeclareOption{merits}{\gdef\@journal{merits}\gdef\@journalfull{Merits}\gdef\@journalshort{Merits}\gdef\@doiabbr{merits}\gdef\@ISSN{2673-8104}\gdef\@continuouspages{yes}}
\DeclareOption{metabolites}{\gdef\@journal{metabolites}\gdef\@journalfull{Metabolites}\gdef\@journalshort{Metabolites}\gdef\@doiabbr{metabo}\gdef\@ISSN{2218-1989}}
\DeclareOption{metals}{\gdef\@journal{metals}\gdef\@journalfull{Metals}\gdef\@journalshort{Metals}\gdef\@doiabbr{met}\gdef\@ISSN{2075-4701}}
\DeclareOption{meteorology}{\gdef\@journal{meteorology}\gdef\@journalfull{Meteorology}\gdef\@journalshort{Meteorology}\gdef\@doiabbr{meteorology}\gdef\@ISSN{2674-0494}\gdef\@continuouspages{yes}}
\DeclareOption{methane}{\gdef\@journal{methane}\gdef\@journalfull{Methane}\gdef\@journalshort{Methane}\gdef\@doiabbr{methane}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{metrology}{\gdef\@journal{metrology}\gdef\@journalfull{Metrology}\gdef\@journalshort{Metrology}\gdef\@doiabbr{metrology}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{micro}{\gdef\@journal{micro}\gdef\@journalfull{Micro}\gdef\@journalshort{Micro}\gdef\@doiabbr{micro}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{microarrays}{\gdef\@journal{microarrays}\gdef\@journalfull{Microarrays}\gdef\@journalshort{Microarrays}\gdef\@doiabbr{microarrays}\gdef\@ISSN{2076-3905}}
\DeclareOption{microbiolres}{\gdef\@journal{microbiolres}\gdef\@journalfull{Microbiology Research}\gdef\@journalshort{Microbiol. Res.}\gdef\@doiabbr{microbiolres}\gdef\@ISSN{2036-7481}\gdef\@continuouspages{yes}}
\DeclareOption{micromachines}{\gdef\@journal{micromachines}\gdef\@journalfull{Micromachines}\gdef\@journalshort{Micromachines}\gdef\@doiabbr{mi}\gdef\@ISSN{2072-666X}}
\DeclareOption{microorganisms}{\gdef\@journal{microorganisms}\gdef\@journalfull{Microorganisms}\gdef\@journalshort{Microorganisms}\gdef\@doiabbr{microorganisms}\gdef\@ISSN{2076-2607}}
\DeclareOption{microplastics}{\gdef\@journal{microplastics}\gdef\@journalfull{Microplastics}\gdef\@journalshort{Microplastics}\gdef\@doiabbr{microplastics}\gdef\@ISSN{2673-8929}\gdef\@continuouspages{yes}}
\DeclareOption{minerals}{\gdef\@journal{minerals}\gdef\@journalfull{Minerals}\gdef\@journalshort{Minerals}\gdef\@doiabbr{min}\gdef\@ISSN{2075-163X}}
\DeclareOption{mining}{\gdef\@journal{mining}\gdef\@journalfull{Mining}\gdef\@journalshort{Mining}\gdef\@doiabbr{mining}\gdef\@ISSN{2673-6489}\gdef\@continuouspages{yes}}
\DeclareOption{modelling}{\gdef\@journal{modelling}\gdef\@journalfull{Modelling}\gdef\@journalshort{Modelling}\gdef\@doiabbr{modelling}\gdef\@ISSN{2673-3951}\gdef\@continuouspages{yes}}
\DeclareOption{molbank}{\gdef\@journal{molbank}\gdef\@journalfull{Molbank}\gdef\@journalshort{Molbank}\gdef\@doiabbr{M}\gdef\@ISSN{1422-8599}}
\DeclareOption{molecules}{\gdef\@journal{molecules}\gdef\@journalfull{Molecules}\gdef\@journalshort{Molecules}\gdef\@doiabbr{molecules}\gdef\@ISSN{1420-3049}}
\DeclareOption{mps}{\gdef\@journal{mps}\gdef\@journalfull{Methods and Protocols}\gdef\@journalshort{Methods Protoc.}\gdef\@doiabbr{mps}\gdef\@ISSN{2409-9279}}
\DeclareOption{msf}{\gdef\@journal{msf}\gdef\@journalfull{Medical Sciences Forum}\gdef\@journalshort{Med. Sci. Forum}\gdef\@doiabbr{msf}\gdef\@ISSN{2673-9992}}
\DeclareOption{mti}{\gdef\@journal{mti}\gdef\@journalfull{Multimodal Technologies and Interaction}\gdef\@journalshort{Multimodal Technol. Interact.}\gdef\@doiabbr{mti}\gdef\@ISSN{2414-4088}}
\DeclareOption{muscles}{\gdef\@journal{muscles}\gdef\@journalfull{Muscles}\gdef\@journalshort{Muscles}\gdef\@doiabbr{muscles}\gdef\@ISSN{2813-0413}\gdef\@continuouspages{yes}}
\DeclareOption{nanoenergyadv}{\gdef\@journal{nanoenergyadv}\gdef\@journalfull{Nanoenergy Advances}\gdef\@journalshort{Nanoenergy Adv.}\gdef\@doiabbr{nanoenergyadv}\gdef\@ISSN{2673-706X}\gdef\@continuouspages{yes}}
\DeclareOption{nanomanufacturing}{\gdef\@journal{nanomanufacturing}\gdef\@journalfull{Nanomanufacturing}\gdef\@journalshort{Nanomanufacturing}\gdef\@doiabbr{nanomanufacturing}\gdef\@ISSN{2673-687X}\gdef\@continuouspages{yes}}
\DeclareOption{nanomaterials}{\gdef\@journal{nanomaterials}\gdef\@journalfull{Nanomaterials}\gdef\@journalshort{Nanomaterials}\gdef\@doiabbr{nano}\gdef\@ISSN{2079-4991}}
\DeclareOption{ncrna}{\gdef\@journal{ncrna}\gdef\@journalfull{Non-coding RNA}\gdef\@journalshort{Non-coding RNA}\gdef\@doiabbr{ncrna}\gdef\@ISSN{2311-553X}}
\DeclareOption{network}{\gdef\@journal{network}\gdef\@journalfull{Network}\gdef\@journalshort{Network}\gdef\@doiabbr{network}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{neuroglia}{\gdef\@journal{neuroglia}\gdef\@journalfull{Neuroglia}\gdef\@journalshort{Neuroglia}\gdef\@doiabbr{neuroglia}\gdef\@ISSN{2571-6980}\gdef\@continuouspages{yes}}
\DeclareOption{neurolint}{\gdef\@journal{neurolint}\gdef\@journalfull{Neurology International}\gdef\@journalshort{Neurol. Int.}\gdef\@doiabbr{neurolint}\gdef\@ISSN{2035-8377}\gdef\@continuouspages{yes}}
\DeclareOption{neurosci}{\gdef\@journal{neurosci}\gdef\@journalfull{NeuroSci}\gdef\@journalshort{NeuroSci}\gdef\@doiabbr{neurosci}\gdef\@ISSN{2673-4087}\gdef\@continuouspages{yes}}
\DeclareOption{nitrogen}{\gdef\@journal{nitrogen}\gdef\@journalfull{Nitrogen}\gdef\@journalshort{Nitrogen}\gdef\@doiabbr{nitrogen}\gdef\@ISSN{2504-3129}\gdef\@continuouspages{yes}}
\DeclareOption{notspecified}{\gdef\@journal{notspecified}\gdef\@journalfull{Journal Not Specified}\gdef\@journalshort{Journal Not Specified}\gdef\@doiabbr{}\gdef\@ISSN{}}
%%\DeclareOption{nri}{\gdef\@journal{nri}\gdef\@journalfull{Natural Resources Informatics}\gdef\@journalshort{Nat. Resour. Inform.}\gdef\@doiabbr{nri}\gdef\@ISSN{2673-981X}\gdef\@continuouspages{yes}}
\DeclareOption{nursrep}{\gdef\@journal{nursrep}\gdef\@journalfull{Nursing Reports}\gdef\@journalshort{Nurs. Rep.}\gdef\@doiabbr{nursrep}\gdef\@ISSN{2039-4403}\gdef\@continuouspages{yes}}
\DeclareOption{nutraceuticals}{\gdef\@journal{nutraceuticals}\gdef\@journalfull{Nutraceuticals}\gdef\@journalshort{Nutraceuticals}\gdef\@doiabbr{nutraceuticals}\gdef\@ISSN{1661-3821}\gdef\@continuouspages{yes}}
\DeclareOption{nutrients}{\gdef\@journal{nutrients}\gdef\@journalfull{Nutrients}\gdef\@journalshort{Nutrients}\gdef\@doiabbr{nu}\gdef\@ISSN{2072-6643}}
\DeclareOption{obesities}{\gdef\@journal{obesities}\gdef\@journalfull{Obesities}\gdef\@journalshort{Obesities}\gdef\@doiabbr{obesities}\gdef\@ISSN{2673-4168}\gdef\@continuouspages{yes}}
\DeclareOption{oceans}{\gdef\@journal{oceans}\gdef\@journalfull{Oceans}\gdef\@journalshort{Oceans}\gdef\@doiabbr{oceans}\gdef\@ISSN{2673-1924}\gdef\@continuouspages{yes}}
\DeclareOption{ohbm}{\gdef\@journal{ohbm}\gdef\@journalfull{Journal of Otorhinolaryngology Hearing and Balance Medicine}\gdef\@journalshort{J. Otorhinolaryngol. Hear. Balance Med.}\gdef\@doiabbr{ohbm}\gdef\@ISSN{2504-463X}}
\DeclareOption{onco}{\gdef\@journal{onco}\gdef\@journalfull{Onco}\gdef\@journalshort{Onco}\gdef\@doiabbr{onco}\gdef\@ISSN{2673-7523}\gdef\@continuouspages{yes}}
%\DeclareOption{oncopathology}{\gdef\@journal{oncopathology}\gdef\@journalfull{}\gdef\@journalshort{}\gdef\@doiabbr{}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{optics}{\gdef\@journal{optics}\gdef\@journalfull{Optics}\gdef\@journalshort{Optics}\gdef\@doiabbr{opt}\gdef\@ISSN{2673-3269}\gdef\@continuouspages{yes}}
\DeclareOption{oral}{\gdef\@journal{oral}\gdef\@journalfull{Oral}\gdef\@journalshort{Oral}\gdef\@doiabbr{oral}\gdef\@ISSN{2673-6373}\gdef\@continuouspages{yes}}
\DeclareOption{organics}{\gdef\@journal{organics}\gdef\@journalfull{Organics}\gdef\@journalshort{Organics}\gdef\@doiabbr{org}\gdef\@ISSN{2673-401X}\gdef\@continuouspages{yes}}
\DeclareOption{organoids}{\gdef\@journal{organoids}\gdef\@journalfull{Organoids}\gdef\@journalshort{Organoids}\gdef\@doiabbr{organoids}\gdef\@ISSN{2674-1172}\gdef\@continuouspages{yes}}
\DeclareOption{osteology}{\gdef\@journal{osteology}\gdef\@journalfull{Osteology}\gdef\@journalshort{Osteology}\gdef\@doiabbr{osteology}\gdef\@ISSN{2673-4036}\gdef\@continuouspages{yes}}
\DeclareOption{oxygen}{\gdef\@journal{oxygen}\gdef\@journalfull{Oxygen}\gdef\@journalshort{Oxygen}\gdef\@doiabbr{oxygen}\gdef\@ISSN{2673-9801}\gdef\@continuouspages{yes}}
\DeclareOption{parasites}{\gdef\@journal{parasites}\gdef\@journalfull{Parasites}\gdef\@journalshort{Parasites}\gdef\@doiabbr{parasites}\gdef\@ISSN{2673-5946}}
\DeclareOption{parasitologia}{\gdef\@journal{parasitologia}\gdef\@journalfull{Parasitologia}\gdef\@journalshort{Parasitologia}\gdef\@doiabbr{parasitologia}\gdef\@ISSN{2673-6772}\gdef\@continuouspages{yes}}
\DeclareOption{particles}{\gdef\@journal{particles}\gdef\@journalfull{Particles}\gdef\@journalshort{Particles}\gdef\@doiabbr{particles}\gdef\@ISSN{2571-712X}\gdef\@continuouspages{yes}}
\DeclareOption{pathogens}{\gdef\@journal{pathogens}\gdef\@journalfull{Pathogens}\gdef\@journalshort{Pathogens}\gdef\@doiabbr{pathogens}\gdef\@ISSN{2076-0817}}
\DeclareOption{pathophysiology}{\gdef\@journal{pathophysiology}\gdef\@journalfull{Pathophysiology}\gdef\@journalshort{Pathophysiology}\gdef\@doiabbr{pathophysiology}\gdef\@ISSN{0928-4680}\gdef\@continuouspages{yes}}
\DeclareOption{pediatrrep}{\gdef\@journal{pediatrrep}\gdef\@journalfull{Pediatric Reports}\gdef\@journalshort{Pediatr. Rep.}\gdef\@doiabbr{pediatric}\gdef\@ISSN{2036-7503}\gdef\@continuouspages{yes}}
\DeclareOption{pharmaceuticals}{\gdef\@journal{pharmaceuticals}\gdef\@journalfull{Pharmaceuticals}\gdef\@journalshort{Pharmaceuticals}\gdef\@doiabbr{ph}\gdef\@ISSN{1424-8247}}
\DeclareOption{pharmaceutics}{\gdef\@journal{pharmaceutics}\gdef\@journalfull{Pharmaceutics}\gdef\@journalshort{Pharmaceutics}\gdef\@doiabbr{pharmaceutics}\gdef\@ISSN{1999-4923}}
\DeclareOption{pharmacoepidemiology}{\gdef\@journal{pharmacoepidemiology}\gdef\@journalfull{Pharmacoepidemiology}\gdef\@journalshort{Pharmacoepidemiology}\gdef\@doiabbr{pharma}\gdef\@ISSN{2813-0618}\gdef\@continuouspages{yes}}
\DeclareOption{pharmacy}{\gdef\@journal{pharmacy}\gdef\@journalfull{Pharmacy}\gdef\@journalshort{Pharmacy}\gdef\@doiabbr{pharmacy}\gdef\@ISSN{2226-4787}}
\DeclareOption{philosophies}{\gdef\@journal{philosophies}\gdef\@journalfull{Philosophies}\gdef\@journalshort{Philosophies}\gdef\@doiabbr{philosophies}\gdef\@ISSN{2409-9287}}
\DeclareOption{photochem}{\gdef\@journal{photochem}\gdef\@journalfull{Photochem}\gdef\@journalshort{Photochem}\gdef\@doiabbr{photochem}\gdef\@ISSN{2673-7256}\gdef\@continuouspages{yes}}
\DeclareOption{photonics}{\gdef\@journal{photonics}\gdef\@journalfull{Photonics}\gdef\@journalshort{Photonics}\gdef\@doiabbr{photonics}\gdef\@ISSN{2304-6732}}
\DeclareOption{phycology}{\gdef\@journal{phycology}\gdef\@journalfull{Phycology}\gdef\@journalshort{Phycology}\gdef\@doiabbr{phycology}\gdef\@ISSN{2673-9410}\gdef\@continuouspages{yes}}
\DeclareOption{physchem}{\gdef\@journal{physchem}\gdef\@journalfull{Physchem}\gdef\@journalshort{Physchem}\gdef\@doiabbr{physchem}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{physics}{\gdef\@journal{physics}\gdef\@journalfull{Physics}\gdef\@journalshort{Physics}\gdef\@doiabbr{physics}\gdef\@ISSN{2624-8174}\gdef\@continuouspages{yes}}
\DeclareOption{physiologia}{\gdef\@journal{physiologia}\gdef\@journalfull{Physiologia}\gdef\@journalshort{Physiologia}\gdef\@doiabbr{physiologia}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{plants}{\gdef\@journal{plants}\gdef\@journalfull{Plants}\gdef\@journalshort{Plants}\gdef\@doiabbr{plants}\gdef\@ISSN{2223-7747}}
\DeclareOption{plasma}{\gdef\@journal{plasma}\gdef\@journalfull{Plasma}\gdef\@journalshort{Plasma}\gdef\@doiabbr{plasma}\gdef\@ISSN{2571-6182}\gdef\@continuouspages{yes}}
\DeclareOption{pollutants}{\gdef\@journal{pollutants}\gdef\@journalfull{Pollutants}\gdef\@journalshort{Pollutants}\gdef\@doiabbr{pollutants}\gdef\@ISSN{2673-4672}\gdef\@continuouspages{yes}}
\DeclareOption{polymers}{\gdef\@journal{polymers}\gdef\@journalfull{Polymers}\gdef\@journalshort{Polymers}\gdef\@doiabbr{polym}\gdef\@ISSN{2073-4360}}
\DeclareOption{polysaccharides}{\gdef\@journal{polysaccharides}\gdef\@journalfull{Polysaccharides}\gdef\@journalshort{Polysaccharides}\gdef\@doiabbr{polysaccharides}\gdef\@ISSN{2673-4176}\gdef\@continuouspages{yes}}
\DeclareOption{poultry}{\gdef\@journal{poultry}\gdef\@journalfull{Poultry}\gdef\@journalshort{Poultry}\gdef\@doiabbr{poultry}\gdef\@ISSN{2674-1164}\gdef\@continuouspages{yes}}
\DeclareOption{powders}{\gdef\@journal{powders}\gdef\@journalfull{Powders}\gdef\@journalshort{Powders}\gdef\@doiabbr{powders}\gdef\@ISSN{2674-0516}\gdef\@continuouspages{yes}}
\DeclareOption{preprints}{\gdef\@journal{preprints}\gdef\@journalfull{Preprints}\gdef\@journalshort{Preprints}\gdef\@doiabbr{}\gdef\@ISSN{}}
\DeclareOption{proceedings}{\gdef\@journal{proceedings}\gdef\@journalfull{Proceedings}\gdef\@journalshort{Proceedings}\gdef\@doiabbr{proceedings}\gdef\@ISSN{2504-3900}}
\DeclareOption{processes}{\gdef\@journal{processes}\gdef\@journalfull{Processes}\gdef\@journalshort{Processes}\gdef\@doiabbr{pr}\gdef\@ISSN{2227-9717}}
\DeclareOption{prosthesis}{\gdef\@journal{prosthesis}\gdef\@journalfull{Prosthesis}\gdef\@journalshort{Prosthesis}\gdef\@doiabbr{prosthesis}\gdef\@ISSN{2673-1592}\gdef\@continuouspages{yes}}
\DeclareOption{proteomes}{\gdef\@journal{proteomes}\gdef\@journalfull{Proteomes}\gdef\@journalshort{Proteomes}\gdef\@doiabbr{proteomes}\gdef\@ISSN{2227-7382}}
\DeclareOption{psf}{\gdef\@journal{psf}\gdef\@journalfull{Physical Sciences Forum}\gdef\@journalshort{Phys. Sci. Forum}\gdef\@doiabbr{psf}\gdef\@ISSN{2673-9984}}
\DeclareOption{psych}{\gdef\@journal{psych}\gdef\@journalfull{Psych}\gdef\@journalshort{Psych}\gdef\@doiabbr{psych}\gdef\@ISSN{2624-8611}\gdef\@continuouspages{yes}}
\DeclareOption{psychiatryint}{\gdef\@journal{psychiatryint}\gdef\@journalfull{Psychiatry International}\gdef\@journalshort{Psychiatry Int.}\gdef\@doiabbr{psychiatryint}\gdef\@ISSN{2673-5318}\gdef\@continuouspages{yes}}
\DeclareOption{psychoactives}{\gdef\@journal{psychoactives}\gdef\@journalfull{Psychoactives}\gdef\@journalshort{Psychoactives}\gdef\@doiabbr{psychoactives}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{publications}{\gdef\@journal{publications}\gdef\@journalfull{Publications}\gdef\@journalshort{Publications}\gdef\@doiabbr{publications}\gdef\@ISSN{2304-6775}}
\DeclareOption{quantumrep}{\gdef\@journal{quantumrep}\gdef\@journalfull{Quantum Reports}\gdef\@journalshort{Quantum Rep.}\gdef\@doiabbr{quantum}\gdef\@ISSN{2624-960X}\gdef\@continuouspages{yes}}
\DeclareOption{quaternary}{\gdef\@journal{quaternary}\gdef\@journalfull{Quaternary}\gdef\@journalshort{Quaternary}\gdef\@doiabbr{quat}\gdef\@ISSN{2571-550X}}
\DeclareOption{qubs}{\gdef\@journal{qubs}\gdef\@journalfull{Quantum Beam Science}\gdef\@journalshort{Quantum Beam Sci.}\gdef\@doiabbr{qubs}\gdef\@ISSN{2412-382X}}
\DeclareOption{radiation}{\gdef\@journal{radiation}\gdef\@journalfull{Radiation}\gdef\@journalshort{Radiation}\gdef\@doiabbr{radiation}\gdef\@ISSN{2673-592X}\gdef\@continuouspages{yes}}
\DeclareOption{reactions}{\gdef\@journal{reactions}\gdef\@journalfull{Reactions}\gdef\@journalshort{Reactions}\gdef\@doiabbr{reactions}\gdef\@ISSN{2624-781X}\gdef\@continuouspages{yes}}
\DeclareOption{receptors}{\gdef\@journal{receptors}\gdef\@journalfull{Receptors}\gdef\@journalshort{Receptors}\gdef\@doiabbr{receptors}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{recycling}{\gdef\@journal{recycling}\gdef\@journalfull{Recycling}\gdef\@journalshort{Recycling}\gdef\@doiabbr{recycling}\gdef\@ISSN{2313-4321}}
\DeclareOption{regeneration}{\gdef\@journal{regeneration}\gdef\@journalfull{Regeneration}\gdef\@journalshort{Regeneration}\gdef\@doiabbr{regeneration}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{religions}{\gdef\@journal{religions}\gdef\@journalfull{Religions}\gdef\@journalshort{Religions}\gdef\@doiabbr{rel}\gdef\@ISSN{2077-1444}}
\DeclareOption{remotesensing}{\gdef\@journal{remotesensing}\gdef\@journalfull{Remote Sensing}\gdef\@journalshort{Remote Sens.}\gdef\@doiabbr{rs}\gdef\@ISSN{2072-4292}}
\DeclareOption{reports}{\gdef\@journal{reports}\gdef\@journalfull{Reports}\gdef\@journalshort{Reports}\gdef\@doiabbr{reports}\gdef\@ISSN{2571-841X}}
\DeclareOption{reprodmed}{\gdef\@journal{reprodmed}\gdef\@journalfull{Reproductive Medicine}\gdef\@journalshort{Reprod. Med.}\gdef\@doiabbr{reprodmed}\gdef\@ISSN{2673-3897}\gdef\@continuouspages{yes}}
\DeclareOption{resources}{\gdef\@journal{resources}\gdef\@journalfull{Resources}\gdef\@journalshort{Resources}\gdef\@doiabbr{resources}\gdef\@ISSN{2079-9276}}
\DeclareOption{rheumato}{\gdef\@journal{rheumato}\gdef\@journalfull{Rheumato}\gdef\@journalshort{Rheumato}\gdef\@doiabbr{rheumato}\gdef\@ISSN{2674-0621}\gdef\@continuouspages{yes}}
\DeclareOption{risks}{\gdef\@journal{risks}\gdef\@journalfull{Risks}\gdef\@journalshort{Risks}\gdef\@doiabbr{risks}\gdef\@ISSN{2227-9091}}
\DeclareOption{robotics}{\gdef\@journal{robotics}\gdef\@journalfull{Robotics}\gdef\@journalshort{Robotics}\gdef\@doiabbr{robotics}\gdef\@ISSN{2218-6581}}
\DeclareOption{ruminants}{\gdef\@journal{ruminants}\gdef\@journalfull{Ruminants}\gdef\@journalshort{Ruminants}\gdef\@doiabbr{ruminants}\gdef\@ISSN{2673-933X}\gdef\@continuouspages{yes}}
\DeclareOption{safety}{\gdef\@journal{safety}\gdef\@journalfull{Safety}\gdef\@journalshort{Safety}\gdef\@doiabbr{safety}\gdef\@ISSN{2313-576X}}
\DeclareOption{sci}{\gdef\@journal{sci}\gdef\@journalfull{Sci}\gdef\@journalshort{Sci}\gdef\@doiabbr{sci}\gdef\@ISSN{2413-4155}}
\DeclareOption{scipharm}{\gdef\@journal{scipharm}\gdef\@journalfull{Scientia Pharmaceutica}\gdef\@journalshort{Sci. Pharm.}\gdef\@doiabbr{scipharm}\gdef\@ISSN{2218-0532}}
\DeclareOption{seeds}{\gdef\@journal{seeds}\gdef\@journalfull{Seeds}\gdef\@journalshort{Seeds}\gdef\@doiabbr{seeds}\gdef\@ISSN{2674-1024}\gdef\@continuouspages{yes}}
\DeclareOption{sensors}{\gdef\@journal{sensors}\gdef\@journalfull{Sensors}\gdef\@journalshort{Sensors}\gdef\@doiabbr{s}\gdef\@ISSN{1424-8220}}
\DeclareOption{separations}{\gdef\@journal{separations}\gdef\@journalfull{Separations}\gdef\@journalshort{Separations}\gdef\@doiabbr{separations}\gdef\@ISSN{2297-8739}}
\DeclareOption{sexes}{\gdef\@journal{sexes}\gdef\@journalfull{Sexes}\gdef\@journalshort{Sexes}\gdef\@doiabbr{sexes}\gdef\@ISSN{2411-5118}\gdef\@continuouspages{yes}}
\DeclareOption{signals}{\gdef\@journal{signals}\gdef\@journalfull{Signals}\gdef\@journalshort{Signals}\gdef\@doiabbr{signals}\gdef\@ISSN{2624-6120}\gdef\@continuouspages{yes}}
\DeclareOption{sinusitis}{\gdef\@journal{sinusitis}\gdef\@journalfull{Sinusitis}\gdef\@journalshort{Sinusitis}\gdef\@doiabbr{sinusitis}\gdef\@ISSN{2309-107X}\gdef\@continuouspages{yes}}
\DeclareOption{skins}{\gdef\@journal{skins}\gdef\@journalfull{Skins}\gdef\@journalshort{Skins}\gdef\@doiabbr{skins}\gdef\@ISSN{}}
\DeclareOption{smartcities}{\gdef\@journal{smartcities}\gdef\@journalfull{Smart Cities}\gdef\@journalshort{Smart Cities}\gdef\@doiabbr{smartcities}\gdef\@ISSN{2624-6511}\gdef\@continuouspages{yes}}
\DeclareOption{sna}{\gdef\@journal{sna}\gdef\@journalfull{Sinusitis and Asthma}\gdef\@journalshort{Sinusitis Asthma}\gdef\@doiabbr{sna}\gdef\@ISSN{2624-7003}}
\DeclareOption{societies}{\gdef\@journal{societies}\gdef\@journalfull{Societies}\gdef\@journalshort{Societies}\gdef\@doiabbr{soc}\gdef\@ISSN{2075-4698}}
\DeclareOption{socsci}{\gdef\@journal{socsci}\gdef\@journalfull{Social Sciences}\gdef\@journalshort{Soc. Sci.}\gdef\@doiabbr{socsci}\gdef\@ISSN{2076-0760}}
\DeclareOption{software}{\gdef\@journal{software}\gdef\@journalfull{Software}\gdef\@journalshort{Software}\gdef\@doiabbr{software}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{soilsystems}{\gdef\@journal{soilsystems}\gdef\@journalfull{Soil Systems}\gdef\@journalshort{Soil Syst.}\gdef\@doiabbr{soilsystems}\gdef\@ISSN{2571-8789}}
\DeclareOption{solar}{\gdef\@journal{solar}\gdef\@journalfull{Solar}\gdef\@journalshort{Solar}\gdef\@doiabbr{solar}\gdef\@ISSN{2673-9941}\gdef\@continuouspages{yes}}
\DeclareOption{solids}{\gdef\@journal{solids}\gdef\@journalfull{Solids}\gdef\@journalshort{Solids}\gdef\@doiabbr{solids}\gdef\@ISSN{2673-6497}\gdef\@continuouspages{yes}}
\DeclareOption{sports}{\gdef\@journal{sports}\gdef\@journalfull{Sports}\gdef\@journalshort{Sports}\gdef\@doiabbr{sports}\gdef\@ISSN{2075-4663}}
\DeclareOption{standards}{\gdef\@journal{standards}\gdef\@journalfull{Standards}\gdef\@journalshort{Standards}\gdef\@doiabbr{standards}\gdef\@ISSN{2305-6703}\gdef\@continuouspages{yes}}
\DeclareOption{stats}{\gdef\@journal{stats}\gdef\@journalfull{Stats}\gdef\@journalshort{Stats}\gdef\@doiabbr{stats}\gdef\@ISSN{2571-905X}\gdef\@continuouspages{yes}}
\DeclareOption{stresses}{\gdef\@journal{stresses}\gdef\@journalfull{Stresses}\gdef\@journalshort{Stresses}\gdef\@doiabbr{stresses}\gdef\@ISSN{2673-7140}\gdef\@continuouspages{yes}}
\DeclareOption{surfaces}{\gdef\@journal{surfaces}\gdef\@journalfull{Surfaces}\gdef\@journalshort{Surfaces}\gdef\@doiabbr{surfaces}\gdef\@ISSN{2571-9637}\gdef\@continuouspages{yes}}
\DeclareOption{surgeries}{\gdef\@journal{surgeries}\gdef\@journalfull{Surgeries}\gdef\@journalshort{Surgeries}\gdef\@doiabbr{surgeries}\gdef\@ISSN{2017-2017}\gdef\@continuouspages{yes}}
\DeclareOption{suschem}{\gdef\@journal{suschem}\gdef\@journalfull{Sustainable Chemistry}\gdef\@journalshort{Sustain. Chem.}\gdef\@doiabbr{suschem}\gdef\@ISSN{2673-4079}\gdef\@continuouspages{yes}}
\DeclareOption{sustainability}{\gdef\@journal{sustainability}\gdef\@journalfull{Sustainability}\gdef\@journalshort{Sustainability}\gdef\@doiabbr{su}\gdef\@ISSN{2071-1050}}
\DeclareOption{symmetry}{\gdef\@journal{symmetry}\gdef\@journalfull{Symmetry}\gdef\@journalshort{Symmetry}\gdef\@doiabbr{sym}\gdef\@ISSN{2073-8994}}
\DeclareOption{synbio}{\gdef\@journal{synbio}\gdef\@journalfull{Synbio}\gdef\@journalshort{Synbio}\gdef\@doiabbr{synbio}\gdef\@ISSN{2674-0583}\gdef\@continuouspages{yes}}
\DeclareOption{systems}{\gdef\@journal{systems}\gdef\@journalfull{Systems}\gdef\@journalshort{Systems}\gdef\@doiabbr{systems}\gdef\@ISSN{2079-8954}}
\DeclareOption{taxonomy}{\gdef\@journal{taxonomy}\gdef\@journalfull{Taxonomy}\gdef\@journalshort{Taxonomy}\gdef\@doiabbr{taxonomy}\gdef\@ISSN{2673-6500}\gdef\@continuouspages{yes}}
\DeclareOption{technologies}{\gdef\@journal{technologies}\gdef\@journalfull{Technologies}\gdef\@journalshort{Technologies}\gdef\@doiabbr{technologies}\gdef\@ISSN{2227-7080}}
\DeclareOption{telecom}{\gdef\@journal{telecom}\gdef\@journalfull{Telecom}\gdef\@journalshort{Telecom}\gdef\@doiabbr{telecom}\gdef\@ISSN{2673-4001}\gdef\@continuouspages{yes}}
\DeclareOption{test}{\gdef\@journal{test}\gdef\@journalfull{Test}\gdef\@journalshort{Test}\gdef\@doiabbr{}\gdef\@ISSN{}}
\DeclareOption{textiles}{\gdef\@journal{textiles}\gdef\@journalfull{Textiles}\gdef\@journalshort{Textiles}\gdef\@doiabbr{textiles}\gdef\@ISSN{2673-7248}\gdef\@continuouspages{yes}}
\DeclareOption{thalassrep}{\gdef\@journal{thalassrep}\gdef\@journalfull{Thalassemia Reports}\gdef\@journalshort{Thalass. Rep.}\gdef\@doiabbr{thalassrep}\gdef\@ISSN{2039-4365}\gdef\@continuouspages{yes}}
\DeclareOption{thermo}{\gdef\@journal{thermo}\gdef\@journalfull{Thermo}\gdef\@journalshort{Thermo}\gdef\@doiabbr{thermo}\gdef\@ISSN{2673-7264}\gdef\@continuouspages{yes}}
\DeclareOption{tomography}{\gdef\@journal{tomography}\gdef\@journalfull{Tomography}\gdef\@journalshort{Tomography}\gdef\@doiabbr{tomography}\gdef\@ISSN{2379-139X}\gdef\@continuouspages{yes}}
\DeclareOption{tourismhosp}{\gdef\@journal{tourismhosp}\gdef\@journalfull{Tourism and Hospitality}\gdef\@journalshort{Tour. Hosp.}\gdef\@doiabbr{tourhosp}\gdef\@ISSN{2673-5768}\gdef\@continuouspages{yes}}
\DeclareOption{toxics}{\gdef\@journal{toxics}\gdef\@journalfull{Toxics}\gdef\@journalshort{Toxics}\gdef\@doiabbr{toxics}\gdef\@ISSN{2305-6304}}
\DeclareOption{toxins}{\gdef\@journal{toxins}\gdef\@journalfull{Toxins}\gdef\@journalshort{Toxins}\gdef\@doiabbr{toxins}\gdef\@ISSN{2072-6651}}
\DeclareOption{transplantology}{\gdef\@journal{transplantology}\gdef\@journalfull{Transplantology}\gdef\@journalshort{Transplantology}\gdef\@doiabbr{transplantology}\gdef\@ISSN{2673-3943}\gdef\@continuouspages{yes}}
\DeclareOption{transportation}{\gdef\@journal{transportation}\gdef\@journalfull{Transportation}\gdef\@journalshort{Transportation}\gdef\@doiabbr{transportation}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{traumacare}{\gdef\@journal{traumacare}\gdef\@journalfull{Trauma Care}\gdef\@journalshort{Trauma Care}\gdef\@doiabbr{traumacare}\gdef\@ISSN{2673-866X}\gdef\@continuouspages{yes}}
\DeclareOption{traumas}{\gdef\@journal{traumas}\gdef\@journalfull{Traumas}\gdef\@journalshort{Traumas}\gdef\@doiabbr{traumas}\gdef\@ISSN{2673-7477}\gdef\@continuouspages{yes}}
\DeclareOption{tropicalmed}{\gdef\@journal{tropicalmed}\gdef\@journalfull{Tropical Medicine and Infectious Disease}\gdef\@journalshort{Trop. Med. Infect. Dis.}\gdef\@doiabbr{tropicalmed}\gdef\@ISSN{2414-6366}}
\DeclareOption{universe}{\gdef\@journal{universe}\gdef\@journalfull{Universe}\gdef\@journalshort{Universe}\gdef\@doiabbr{universe}\gdef\@ISSN{2218-1997}}
\DeclareOption{urbansci}{\gdef\@journal{urbansci}\gdef\@journalfull{Urban Science}\gdef\@journalshort{Urban Sci.}\gdef\@doiabbr{urbansci}\gdef\@ISSN{2413-8851}}
\DeclareOption{uro}{\gdef\@journal{uro}\gdef\@journalfull{Uro}\gdef\@journalshort{Uro}\gdef\@doiabbr{uro}\gdef\@ISSN{2673-4397}\gdef\@continuouspages{yes}}
\DeclareOption{vaccines}{\gdef\@journal{vaccines}\gdef\@journalfull{Vaccines}\gdef\@journalshort{Vaccines}\gdef\@doiabbr{vaccines}\gdef\@ISSN{2076-393X}}
\DeclareOption{vehicles}{\gdef\@journal{vehicles}\gdef\@journalfull{Vehicles}\gdef\@journalshort{Vehicles}\gdef\@doiabbr{vehicles}\gdef\@ISSN{2624-8921}\gdef\@continuouspages{yes}}
\DeclareOption{venereology}{\gdef\@journal{venereology}\gdef\@journalfull{Venereology}\gdef\@journalshort{Venereology}\gdef\@doiabbr{venereology}\gdef\@ISSN{2674-0710}\gdef\@continuouspages{yes}}
\DeclareOption{vetsci}{\gdef\@journal{vetsci}\gdef\@journalfull{Veterinary Sciences}\gdef\@journalshort{Vet. Sci.}\gdef\@doiabbr{vetsci}\gdef\@ISSN{2306-7381}}
\DeclareOption{vibration}{\gdef\@journal{vibration}\gdef\@journalfull{Vibration}\gdef\@journalshort{Vibration}\gdef\@doiabbr{vibration}\gdef\@ISSN{2571-631X}\gdef\@continuouspages{yes}}
\DeclareOption{virtualworlds}{\gdef\@journal{virtualworlds}\gdef\@journalfull{Virtual Worlds}\gdef\@journalshort{Virtual Worlds}\gdef\@doiabbr{virtualworlds}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{viruses}{\gdef\@journal{viruses}\gdef\@journalfull{Viruses}\gdef\@journalshort{Viruses}\gdef\@doiabbr{v}\gdef\@ISSN{1999-4915}}
\DeclareOption{vision}{\gdef\@journal{vision}\gdef\@journalfull{Vision}\gdef\@journalshort{Vision}\gdef\@doiabbr{vision}\gdef\@ISSN{2411-5150}}
\DeclareOption{waste}{\gdef\@journal{waste}\gdef\@journalfull{Waste}\gdef\@journalshort{Waste}\gdef\@doiabbr{waste}\gdef\@ISSN{2813-0391}\gdef\@continuouspages{yes}}
\DeclareOption{water}{\gdef\@journal{water}\gdef\@journalfull{Water}\gdef\@journalshort{Water}\gdef\@doiabbr{w}\gdef\@ISSN{2073-4441}}
\DeclareOption{wem}{\gdef\@journal{wem}\gdef\@journalfull{Wildlife Ecology and Management}\gdef\@journalshort{Wildl. Ecol. Manag.}\gdef\@doiabbr{}\gdef\@ISSN{1234-4321}}
\DeclareOption{wevj}{\gdef\@journal{wevj}\gdef\@journalfull{World Electric Vehicle Journal}\gdef\@journalshort{World Electr. Veh. J.}\gdef\@doiabbr{wevj}\gdef\@ISSN{2032-6653}}
\DeclareOption{wind}{\gdef\@journal{wind}\gdef\@journalfull{Wind}\gdef\@journalshort{Wind}\gdef\@doiabbr{wind}\gdef\@ISSN{2674-032X}\gdef\@continuouspages{yes}}
\DeclareOption{women}{\gdef\@journal{women}\gdef\@journalfull{Women}\gdef\@journalshort{Women}\gdef\@doiabbr{women}\gdef\@ISSN{2673-4184}\gdef\@continuouspages{yes}}
\DeclareOption{world}{\gdef\@journal{world}\gdef\@journalfull{World}\gdef\@journalshort{World}\gdef\@doiabbr{world}\gdef\@ISSN{2673-4060}\gdef\@continuouspages{yes}}
\DeclareOption{youth}{\gdef\@journal{youth}\gdef\@journalfull{Youth}\gdef\@journalshort{Youth}\gdef\@doiabbr{youth}\gdef\@ISSN{2673-995X}\gdef\@continuouspages{yes}}
\DeclareOption{zoonoticdis}{\gdef\@journal{zoonoticdis}\gdef\@journalfull{Zoonotic Diseases}\gdef\@journalshort{Zoonotic Dis.}\gdef\@doiabbr{zoonoticdis}\gdef\@ISSN{2813-0227}\gdef\@continuouspages{yes}}


==> response_letter.tex <==
\begin{center}
\large
\textbf{Response to Reviewers' Comments}
\end{center}

\begin{center}
Ms. Ref. No.: PHOTO-D-22-00486

ISPRS Journal of Photogrammetry and Remote Sensing
\end{center}

\bigbreak

\begin{flushleft}
\textbf{Dear Editor:}
\end{flushleft}

\textbf{Thank you very much for handling our manuscript. We appreciate the time and efforts from you and the Reviewers who provided us with the opportunity to improve the manuscript based on the insightful comments and suggestions. These comments and suggestions are highly valuable for us to improve this work. We have carefully revised the manuscript. Our responses to Reviewers' comments are detailed below point by point in bold type font. Revised sentences are coloured in blue in this response letter, and highlighted in yellow background in the revised manuscript.}

\bigbreak

\textbf{\underline{Response to Reviewer 1's comments:}}

Reviewer 1: In this study, the authors assessed the potential of DESIS hyperspectral data to predict species richness over two regions of Australia by testing the best combination of three feature extraction procedures (PCA, CCA, and PLS) and three regression models (OLSR, GPR, and KRR). Furthermore, they compared the predictive performance of the DESIS model with that derived from the MSI/Sentinel-2 data.

Overall, the contribution of the work to the literature is not clear, which is aggravated by the absence of a Discussion section. The manuscript has also problems of structure with some results being presented in Methodology. One of my major criticisms is the perception of a mere statistical study without support of a robust spectral discussion on the differences in species richness of sample plots or classes. For instance, reflectance spectra showing the differences on each region between low and high species-richness classes are never shown in the manuscript. This is essential to understand all the analyses. The authors should clearly mention plot size (20 x 20 m?) and assume the constraints of using 30-m spatial resolution data in the analysis. The authors conclude that the best predictions were obtained with PLS and GPR. However, looking at Tables 2 and 3, we observed small differences in r and RMSE values across feature extraction techniques and regression models. This aspect should be at least highlighted in Conclusions. Finally, additional work is necessary to simulate MSI/Sentinel-2 from DESIS to support the discussion on the influence of spectral resolution on predictions.

I recommend Major Revision for this submission. The major comments that deserve attention in a revised version are described below.

\textbf{Re: Thank you very much for your careful review, and the insightful comments and suggestions. These comments and suggestions are highly valuable for us to improve this work. We have carefully revised the manuscript, with detailed revisions being listed below point by point in bold type font. Revised sentences are coloured in blue in this response letter, and highlighted in yellow background in the revised manuscript.}

\bigbreak

1. Title and objectives of the manuscript: Although not clearly stated for the readers, the main objective of the work is to test the combination of different feature extraction procedures (PCA, CCA, and PLS) and regression models (OLSR, GPR, and KRR) for the predictive performance of species richness in Australia using DESIS data. The title of the work should be revisited and modified to clarify this point. The same comment is valid for the general and specific objectives.

\textbf{Re: The authors would like to thank the Reviewer for the helpful comment. As pointed out by the Reviewer, the main objective of our study is to test and compare several combinations of feature extraction procedures and regression models in predicting plant species richness from DESIS hyperspectral data. In order to clarify this objective, we have modified the title of this work. Relevant statements have been added in the Abstract, Introduction, and Conclusion sections. Detailed revisions are listed as follows:}

\textbf{(1) We have modified the title of the manuscript in order to highlight the main objective of this work:}

\textbf{New Title: \textcolor{blue}{``Plant Species Richness Prediction from DESIS Hyperspectral Data: A Comparison Study on Feature Extraction Procedures and Regression Models"}}

\textbf{(2) In the Abstract section, the following sentence has been added to clarify the feature extraction procedures and regression models being tested in our study:}

\textbf{In Abstract: \textcolor{blue}{``We tested and compared the effectiveness of Principal Component Analysis (PCA), Canonical Correlation Analysis (CCA), and Partial Least Squares analysis (PLS) for feature extraction, and Ordinary Least Squares Regression (OLSR), Kernel Ridge Regression (KRR), and Gaussian Process Regression (GPR) for regression."}}

\textbf{(3) In the Introduction section, the following sentence has been added:}

\textbf{Lines 89--92: \textcolor{blue}{``We tested the combination of different feature extraction procedures (PCA, CCA, and PLS) and regression models (OLSR, GPR, and KRR) for the predictive performance of species richness with DESIS data."}}

\textbf{(4) In the Conclusion section, the following sentence has been added:}

\textbf{Lines 526--527: \textcolor{blue}{``We evaluated the performance of several combinations of feature extraction procedures (PCA, CCA, and PLS) and regression models (OLSR, KRR, and GPR)."}}

\bigbreak

2. It is important to separate Results from Discussion. Please, insert a Discussion section. In the first paragraph of Discussion, clearly mention the novel components of the work when compared to previous papers published on the topic. The use of a new sensor is not enough for publication. How do your findings add to the literature? Part of the Discussion section is wrongly positioned in the last two sections of Results.

\textbf{Re: We would like to thank the Reviewer for the insightful comment. In the revised manuscript, we have inserted a dedicated Discussions section which is separate from the Results section. In the Discussions section, we have clarified and highlighted the novel components of our study in comparison with previous works.}

\textbf{Compared with previous studies, we make use of all available bands to extract spectral features, rather than selecting pre-defined features that usually incorporate information from a subset of the bands. This distinguishes our work from earlier studies on the same topic. The following paragraph has been added in the Discussions section in order to highlight this point:}

\textbf{Lines 424--434: \textcolor{blue}{``Obtaining informative features from hyperspectral data is important to the success of subsequent interference of plant species richness. In previous studies, features have been primarily selected as a subset of the original bands, or as spectral indices computed from a subset of the original bands (e.g., \cite{malhi2020synergetic}, \cite{peng2018assessment}, and \cite{wang2016seasonal}). The bands or indices are often selected based on our \emph{a priori} knowledge of the spectral properties, such as absorption features of biochemical contents. Though selected features usually offer good explainability, it means we have to discard information in unselected bands. Considering the large number of bands in hyperspectral data, many of them would be discarded as the high collinearity of hyperspectral data often requires a considerable reduction of dimensionality. In contrast, the feature extraction approach, as adopted in this work, makes use of the information in all original bands by transforming them into a new feature space of lower and non-collinear dimensionality."}}

\textbf{Another component that distinguishes our work from previous studies is that a novel kernel function is proposed to account for both linear and non-linear patterns in the relationship between spectral features and species richness. The following discussion has been added in the revised manuscript:}

\textbf{Lines 435--442: \textcolor{blue}{``Linear models have been primarily employed in previous studies to relate features to species richness. For example, multiple linear regression has been adopted by \cite{wang2016seasonal} and \cite{malhi2020synergetic}, and stepwise linear regression by \cite{peng2018assessment}. However, the relationship between features and richness might not necessarily  follows simply a linear pattern. In our study, a novel kernel function is proposed (Eq. \ref{eq:kernel_function}), with the dot-product and radial-basis function kernels account for the linearity and non-linearity of the data, respectively, and the white kernel explains the noise in the data. The ability of our model to explore both linear and non-linear patterns distinguishes our work from aforementioned studies."}}

\bigbreak

3. I particularly had difficulties to understand the reason for using feature extraction procedures instead of feature selection approaches, which would pick the best reflectance bands of DESIS to be used as input data in the regression models. If one the objectives is to detect the best spectral intervals for predicting species richness, feature selection would be a better alternative than feature extraction. Anyway, the authors should at least justify in Introduction the choice of this feature extraction approach when compared to the feature selection alternative. What are advantages of transforming data for regression modelling (feature extraction versus feature selection discussion)?

\textbf{Re: We agree with the Reviewer that it is necessary to justify the use of feature extraction procedures. In the revised manuscript, we have added the following sentences in the Introduction section, in order to explain the merit of feature extraction as compared to feature selection:}

\textbf{Line 66--73: \textcolor{blue}{``In contrast to feature selection that chooses a subset of the original bands (or spectral indices computed from a subset of the original bands), feature extraction techniques such as PCA, CCA, and PLS are able to makes use of information in all bands by transforming them into compact yet informative features. Compared with pre-defined vegetation indices such as Ratio Vegetation Index (RVI) and Normalized Difference Vegetation Index (NDVI), spectral features generated with feature extraction have shown better performance in extracting useful information from hyperspectral measurements \citep{zhao2014earlya}."}}

\textbf{A discussion on feature extraction vs. feature selection has been added into the Discussions section:}

\textbf{Lines 424--434: \textcolor{blue}{``Obtaining informative features from hyperspectral data is important to the success of subsequent interference of plant species richness. In previous studies, features have been primarily selected as a subset of the original bands, or as spectral indices computed from a subset of the original bands (e.g., \cite{malhi2020synergetic}, \cite{peng2018assessment}, and \cite{wang2016seasonal}). The bands or indices are often selected based on our \emph{a priori} knowledge of the spectral properties, such as absorption features of biochemical contents. Though selected features usually offer good explainability, it means we have to discard information in unselected bands. Considering the large number of bands in hyperspectral data, many of them would be discarded as the high collinearity of hyperspectral data often requires a considerable reduction of dimensionality. In contrast, the feature extraction approach, as adopted in this work, makes use of the information in all original bands by transforming them into a new feature space of lower and non-collinear dimensionality."}}

\textbf{Thank you very much for this valuable comment!}

\bigbreak

4. I recommend that the authors revisit the structure of the text. For instance, section 2 is Material and Methods. However, it includes unnecessarily some results that should be moved to the Results section. Figure 3 does not add for the comprehension of the text. Please, delete it. You should replace it by a figure showing reflectance differences on each region between low, intermediate and high species richness plots.

\textbf{Re: We would like to thank the Reviewer for helpful comment. The structure of manuscript has been revisited. Wrongly placed materials have now been restructured into appropriate positions. As suggested, Figure 3 has been deleted, and it has been replaced with a new figure showing reflectance differences between low, intermediate and high species richness plots. The new figure is placed into the Results section, along with added text to illustrate and explain the figure. The new figure and text are:}

\textbf{Lines 309--323:} 

\subsection*{\textbf{\textcolor{blue}{``3.1. Spectral Reflectance Differences Between Species Richness Classes}}}

\textcolor{blue}{\textbf{The blue, green and red curves in Fig. \ref{fig:different_richness} show the DESIS spectra averaged over ground sampling plots with species richness falling into the low, intermediate, and high tertiles, respectively. Results for the Southern Tablelands and Snowy Mountains regions are displayed in Figs \ref{fig:different_richness}a and b, respectively. For each region, it was observed that plots of higher richness showed a lower reflectance in the visible range of $400\sim680$ nm. Considering that major absorption features of chlorophyll are located within the visible region \citep{zhao2014earlya}, the lower reflectance in this spectral portion might indicate a higher concentration of chlorophyll. It was also observed that plots of higher richness showed a higher reflectance in the near-infrared plateau of $780\sim1000$ nm and a steeper red edge between $680\sim780$ nm, which might suggest a larger Leaf Area Index (LAI) \citep{delegido2013red} and a greater vegetation vigor \citep{boochs1990shape} for those plots. On the basis of these observations, the spectral shape of high richness plots, as compared with spectra of intermediate and low richness plots, may imply a generally richer vegetation. This is consistent with findings reported in literature that high species richness enhances primary productivity \citep{wang2016seasonal, grace2016integrative} and biomass \citep{malhi2020synergetic, tilman1997influence}."}}

\begin{figure}[H]
\centering
\captionsetup{font=footnotesize}
\includegraphics[width=9cm]{figures/different_richness.jpg}
\caption*{\textcolor{blue}{Figure 4: Average DESIS reflectance spectra calculated from field sample plots with low, intermediate, and high species richness for the (a) Southern Tablelands and (b) Snowy Mountains regions.}}
\end{figure}

\bigbreak

5. Maybe you should consider the insertion of a new sub-section in Results (something like "Spectral reflectance differences between the species richness classes"). It is very important to insert average DESIS reflectance spectra calculated from field sample plots with low, intermediate, and high species richness, as observed for both sites in Figure 2. Again, this is very important to understand the consistency of the statistical modelling and anticipate the best spectral intervals for predicting species richness. You should agree that 30-m spatial resolution is not the best scale to predict species richness, which generally requires high spatial and spectral resolution data.

\textbf{Re: As suggested by the Reviewer, we have added a new subsection in the revised manuscript, titled \textcolor{blue}{``Spectral Reflectance Differences Between Species Richness Classes"}. A new figure has been inserted into this new subsection, showing the average DESIS reflectance spectra calculated from field sample plots with low, intermediate, and high species richness. Please refer to our response to the previous point (Comment 4) for the newly inserted subsection and figure.}

\textbf{We agree with the Reviewer that, compared to hyperspectral data of higher spatial resolutions, it is challenging to predict species richness with the 30-m spatial resolution of DESIS. The following sentences are added in the Introduction in order to highlight this point:}

\textbf{Lines 52--57: \textcolor{blue}{``It is worth noting the added challenge of spaceborne hyperspectral imagery such as DESIS having a larger pixel size (30m) than typical airborne (ranging from a few centimeters to several meters). As the signal of a large pixel tends to comprise a mix of multiple species, many techniques previously used to quantify richness with hyperspectral data, which detect individual species and then sum up to get richness (e.g., \cite{asner2008hyperspectral,jeanbaptiste2014}), cannot be applied."}}

\textbf{Many thanks for the valuable comment!}

\bigbreak

6. Another problem in the work is the comparison between DESIS and MSI/Sentinel-2 results. In section 3.5, the discussion on the comparison between DESIS and MSI/Sentinel-2 is not entirely correct. The comparison is not fair considering the differences in instrument specifications and geometry of data acquisition. To confirm that spectral resolution is the main factor explaining the differences in predictive performance of species richness, the authors should simulate the MSI response from DESIS data using the MSI/Sentinel-2 filter functions. This is easy to do and can be quickly implemented. By adopting this strategy, the comparison between the two instruments in terms of spectral resolution will be fair. In Figures 10a and 10b, in addition to the results of the original MSI/Sentinel-2, you could insert the fitting lines and statistics for the simulated MSI data from DESIS. It will strength the discussion of results.

\textbf{Re: We agree with the Reviewer that it is important to conduct a fair comparison between hyperspectral and multispectral data. As suggested by the Reviewer, we have simulated a Sentinel-2-like synthetic data set by resampling the DESIS spectra with Sentinel-2's spectral response functions. The following sentences have been added in the revised manuscript:}

\textbf{Lines 301--307: \textcolor{blue}{``In order to conduct a fair comparison between hyperspectral and multispectral data with minimised differences in instrumental specifications and acquisition conditions, a Sentinel-2-like synthetic data set was simulated from the DESIS data. The simulation involved resampling the DESIS spectra using the spectral response functions of Sentinel-2's visible and near-infrared bands. Both the real and synthetic Sentinel-2 sets were used for species richness prediction, with results being compared to those achieved with DESIS data."}}

\textbf{A new figure has been inserted in the Results section to present the results achieved with the Sentinel-2-like synthetic data set:}

\begin{figure}[H]
\centering
\includegraphics[width=9cm]{figures/synthetic.jpg}
\captionsetup{font=footnotesize}
\caption*{\textcolor{blue}{Figure 12: Correlation diagrams between the ground-truth species richness and values predicted from the Sentinel-2-like synthetic multispectral data set for the (a) Southern Tablelands and (b) Snowy Mountains regions. The $r$ and RMSE stand for the coefficient of correlation and root-mean-square error.}}
\end{figure}

\textbf{Many thanks for the helpful suggestion!}

\bigbreak

7. The authors used three feature extraction procedures but did not discuss in depth the results. In section 3.1, the authors defined the hyperparameters based on the accuracy of the predicted richness. However, it is important to strength this section with more statistical results from the three techniques (PCA, CCA, and PLS) used for feature extraction. For instance, the authors could include a table showing the component matrix loadings from PCA (e.g., first five components) and the eigenvalues, indicating the variance explained by each component (and also the cumulative variance). What is the cumulative variance retained by the first two or three principal components? We generally use this criterion (cumulative variance or eigenvalues greater than one) to define the number of components to be retained in the analysis. What represents the first two principal components? Is the first principal component showing vegetation brightness variations? Please, look at the eigenvectors to understand their meaning. In short, add tables to reinforce the statistical analysis of PCA, CCA, and PLS and to understand the meaning of the first components shown in Figure 5 or retained in the analysis. Strength section 3.1.

\textbf{Re: We would like to thank the Reviewer for the highly helpful comment. In the revised manuscript, we have strengthened the results in Section 3.1 (now indexed as Section 3.2 in the revised manuscript) as per the Reviewer's suggestion. A table has been added to show to the eigenvalue, explained variance, and cumulative percentage of explained variance for different components. A figure has been added to depict the shapes of selected components. Sentences have been added in the text in order to illustrate the new table and figure. Detailed revisions are listed below.}

\textbf{(1) A new table (Table 2) has been added to show the eigenvalue, percentage of explained variance, and cumulative percentage of explained variance for components produced with Principal Component Analysis (PCA), Canonical Correlation Analysis (CCA), and Partial Least Squares analysis (PLS). The added table is:}

\begin{table}[H]
\scriptsize
\caption*{\textcolor{blue}{Table 2: The eigenvalue, percentage of explained variance, and cumulative percentage of explained variance for components produced with Principal Component Analysis (PCA), Canonical Correlation Analysis (CCA), and Partial Least Squares analysis (PLS).}}
\renewcommand{\arraystretch}{1.1}
{\color{blue}
\begin{tabular}{cccccccccc}
\toprule
\multirow{2}{*}{Component} & \multicolumn{3}{c}{PCA} & \multicolumn{3}{c}{CCA} & \multicolumn{3}{c}{PLS} \\
& \multicolumn{1}{c}{Eigenvalue} & \multicolumn{1}{c}{\shortstack{\% of \\ Variance}} & \multicolumn{1}{c}{\shortstack{Cumulative \% \\ of Variance}} & \multicolumn{1}{c}{Eigenvalue} & \multicolumn{1}{c}{\shortstack{\% of \\ Variance}} & \multicolumn{1}{c}{\shortstack{Cumulative \% \\ of Variance}} & \multicolumn{1}{c}{Eigenvalue} & \multicolumn{1}{c}{\shortstack{\% of \\ Variance}} & \multicolumn{1}{c}{\shortstack{Cumulative \% \\ of Variance}} \\ 
\hline
1 &44.35 &84.48 &84.48 &40.43 &74.61 &74.61 &40.96 &75.58 &75.58 \\
2 &4.90 &9.34 &93.81 &7.98 &14.73 &89.34 &6.39 &11.80 &87.38 \\
3 &2.22 &4.23 &98.04 &4.16 &7.67 &97.01 &4.94 &9.12 &96.50 \\
4 &0.44 &0.84 &98.87 &0.61 &1.13 &98.14 &0.70 &1.29 &97.79 \\
5 &0.22 &0.41 &99.29 &0.48 &0.89 &99.03 &0.41 &0.75 &98.55 \\
6 &0.10 &0.18 &99.47 &0.12 &0.23 &99.26 &0.23 &0.42 &98.97 \\
7 &0.04 &0.08 &99.55 &0.10 &0.19 &99.45 &0.14 &0.26 &99.22 \\
8 &0.04 &0.08 &99.63 &0.08 &0.14 &99.59 &0.11 &0.19 &99.42 \\
9 &0.03 &0.06 &99.69 &0.06 &0.11 &99.69 &0.08 &0.14 &99.56 \\
10 &0.02 &0.04 &99.73 &0.04 &0.08 &99.77 &0.06 &0.11 &99.67 \\ 
\bottomrule
\end{tabular}}
\end{table}

\textbf{(2) A new figure (Figure 6) has been added to depict the first and second components that have been chosen for regression in our study. The added figure is:}

\begin{figure}[H]
\centering
\captionsetup{font=footnotesize}
\includegraphics[width=11cm]{figures/components.jpg}
\caption*{\textcolor{blue}{Figure 6: The first and second components for the transformed DESIS spectra. Left column: Result for the Southern Tablelands with (a) Principal Component Analysis (PCA), (b) Canonical Correlation Analysis (CCA), and (c) Partial Least Squares analysis (PLS); Right column: Result for the Snowy Mountains region with (d) PCA, (e) CCA, and (f) PLS.}}
\end{figure}

\textbf{(3) The following sentences have been added in order to illustrate the new table and figure:}

\textbf{Lines 332--335: \textcolor{blue}{``The eigenvalue, percentage of explained variance, and cumulative percentage of explained variance with different components are shown in Table \ref{tab:eigen}. It was seen that with two components, the PCA, CCA, and PLS could explain 93.81$\%$, 89.34$\%$, and 87.38$\%$ of variance in the DESIS data, respectively."}}

\textbf{Lines 337--339: \textcolor{blue}{``The first and second components are plotted in Fig. \ref{fig:component_12}. The first component depicted the general shape of the spectral brightness, while the second component highlighted the more on local spectral features of the spectrum."}}

\textbf{Thanks for the insightful comment!}

\bigbreak

8. Methodology (L135): More details on the atmospheric correction of DESIS data are necessary. Was it based on a physical model? What was the strategy used for estimating visibility? What was the atmospheric model? Please, provide more details on the conversion of radiance data into surface reflectance images.

\textbf{Re: We agree with the Reviewer that it is essential to provide details on the correction of atmospheric effects in DESIS data. The conversion of radiance data into surface reflectance images involves applying atmospheric correction within DLR’s PACO (Python Atmospheric COrrection) software \citep{de2018validation}. The MODTRAN\textsuperscript{\textregistered} radiative transfer model \citep{berkmodtran} is used for simulating atmospheric effects. Aerosol optical thickness and water vapour content are retrieved per pixel using reflectance in the red and NIR bands, and bands around the water absorption features of 820 nm, respectively. In the revised manuscript, the following description has been added to clarify the procedure being applied for atmospheric correction in DESIS data:}

\textbf{Lines 148--154: \textcolor{blue}{``In our study, the DESIS Level-2A product was used. It consisted of surface reflectance images with atmospheric correction having been applied. The correction was conducted with DLR's PACO (Python Atmospheric COrrection) software \mbox{\citep{de2018validation}} where the MODTRAN\textsuperscript{\textregistered} radiative transfer model \mbox{\citep{berkmodtran}} served as the module for simulating atmospheric effects. As inputs for atmospheric simulation, aerosol optical thickness and water vapour content were retrieved per pixel using reflectance in the red and NIR bands, and bands around the water absorption features of 820 nm, respectively."}}

\bigbreak

9. Methodology (Lines 145-147): It seems that DESIS is a large FOV system. Therefore, the view zenith angle varies along- and across-track, as mentioned by the authors. The authors describe a mean-data normalization to compensate for bidirectional effects. I particularly had difficulties to understand this approach. The authors should at least include support of literature for this approach, which sounds very empirical to me. Was this approach used in other studies to correct BRDF effects?

\textbf{Re: As pointed out by the Reviewer, the DESIS instrument has a wide viewing angle, which is a result of the $4.1^{\circ}$ field of view in conjunction with the $\pm15^{\circ}$ along track pointing capability of the DESIS sensor, and the $\pm25^{\circ}$ along track and $-45^{\circ}$ $\sim$ $+5^{\circ}$ cross track tilting capability of the MUSES platform. Therefore, it is important to correct the BRDF effects in DESIS data. The following sentence has been added in the revised manuscript in order to highlight the wide viewing angle of the DESIS system:}

\textbf{Lines 163--166: \textcolor{blue}{``The Bidirectional Reflectance Distribution Function (BRDF) effect in DESIS data is unneglectable, given the $4.1^{\circ}$ field of view in conjunction with the $\pm15^{\circ}$ along track pointing capability of the DESIS sensor, and the $\pm25^{\circ}$ along track and $-45^{\circ}$ $\sim$ $+5^{\circ}$ cross track tilting capability of the MUSES platform."}}

\textbf{The approach to correct the BRDF effect in our study involves dividing the value in each spectral band by the mean value over all bands. This approach has been adopted in \cite{green1985analysis} and \cite{ong2014mapping} to correct airborne hyperspectral data that suffers from directional variations because of the topographic relief of the study area and the BRDF effect of the ground target. As suggested, we have added aforementioned studies as references in the revised manuscript:}

\textbf{Lines 166--169: \textcolor{blue}{``Following the approach adopted in \cite{green1985analysis} and \cite{ong2014mapping} for correcting BRDF effect in hyperspectral data, in our study each DESIS spectra was mean-normalised with each spectral band being divided by the mean value over all bands."}}

\textbf{Many thanks for the valuable suggestion!}

\bigbreak

10. In line 135, pleas, insert a more complete description of the DESIS instrument. Is it a large FOV sensor? What is the radiometric resolution and signal-to-noise? How does this spectrometer work?

\textbf{Re: We would like to thank the Reviewer for the helpful suggestion. We agree that a more comprehensive description of the DESIS instrument and its specifications will provide readers with a better understanding of the hyperspectral data set that we have applied in this work. As suggested, a new paragraph has been inserted in the revised manuscript to describe DESIS specifications including the radiometric resolution, signal-to-noise ratio, and operation mode of the sensor:}

\textbf{Lines 141--147: \textcolor{blue}{``The DESIS spectrometer \citep{krutz2019instrument} is embedded in the MUSES platform onboard the International Space Station at an altitude of approximately 400 km. It operates in a push-broom imaging mode featuring state-of-the-art radiometric and spectral specifications. It delivers hyperspectral images with 235 spectral bands over the visible and near-infrared regions of 400 $\sim$ 1000 nm, with a spectral resolution of 2.55 nm and a spatial resolution of 30 m. The radiometric resolution for each band is 12 bit with 1 bit gain. The signal-to-noise ratio is 195 at the wavelength of 550 nm."}}

\textbf{The field of view and pointing capability of the DESIS instrument, as well as the tilting capability of the MUSES platform, have also been clarified in the revised manuscript:}

\textbf{Lines 163--166: \textcolor{blue}{``The Bidirectional Reflectance Distribution Function (BRDF) effect in DESIS data is unneglectable, given the $4.1^{\circ}$ field of view in conjunction with the $\pm15^{\circ}$ along track pointing capability of the DESIS sensor, and the $\pm25^{\circ}$ along track and $-45^{\circ}$ $\sim$ $+5^{\circ}$ cross track tilting capability of the MUSES platform."}}

\bigbreak

11. In Figure 9, for the consistency of analysis, it is important to show the results for the other techniques (or at least for PCA). Please, inspect the component matrix loadings results from PCA, which expresses the correlation between each band and a given component. In Figure 9, plot the results for PCA and compare the spectral intervals indicated as the most important to predict species reachness by both techniques. Do the same for CCA, if possible.

\textbf{Re: In the revised manuscript, we have added the PCA and CCA results to this figure. Thanks for valuable suggestion! The new figure is:}

\begin{figure}[H]
\centering
\includegraphics[width=11cm]{figures/sensitivity_new.jpg}
\captionsetup{font=footnotesize}
\caption*{\textcolor{blue}{Figure 10: Relative importance analysis for the DESIS bands in predicting plant species richness with spectral features being extracted by (a) Principal Component Analysis (PCA), (b) Canonical Correlation Analysis (CCA), and (c) Partial Least Squares analysis (PLS).}}
\end{figure}

\bigbreak

12. In Figure 9, delete the decimal places and use regularly spaced wavelengths to represent your results. The DESIS bands were downsampled to 10 nm and the idea here was to discuss spectral intervals instead of specific bands.

\textbf{Re: As suggested, we have improved this figure by replacing the decimal places with regularly spaced wavelengths. Please refer to our response to the previous comment (Comment 11) for the updated figure. Thanks!}

\bigbreak

13. Conclusions: Caution is necessary here. In fact, differences in r and RMSE values were low across feature extraction techniques and regression models. For instance, the RMSE ranged from 5.89 to 6.08 for the Southern Tablelands region (Table 2), and from 5.97 to 6.24 for the Snowy Mountains region (Table 3). The authors should highlight this aspect before describing the performance of PLS with GPR as the best one.

\textbf{Re: In the revised manuscript, we have added a sentence in order to highlight the low differences among feature extraction techniques and regression models. Thanks for the suggestion! The added sentence is:}

\textbf{Lines 530--531: \textcolor{blue}{``Prediction accuracies fell within a comparable range for different combinations of feature extraction techniques and regression models (Tables 2 and 3)."}}

\bigbreak

Other comments:

- L39: REF?

\textbf{Re: We would like to thank the Reviewer for pointing out this issue. In the revised manuscript, it has been replaced with the correct references. The revised sentence is:}

\textbf{Lines 37--40: \textcolor{blue}{``Most research into the relationships between biodiversity and hyperspectral data have made use of hand-held or airborne hyperspectral sensors, which are more readily available than spaceborne hyperspectral data-streams (e.g., \cite{peng2018assessment}, \cite{asner2008hyperspectral}, \cite{jeanbaptiste2014}, and \cite{hacker2020retrieving})."}}

\bigbreak

- L120: Please, replace ``plot size" by ``plot area". Is it plot size 20 x 20 m? The same comment for Table 1.

\textbf{Re: Many thanks for the suggestion! In the revised manuscript, we have replaced ``plot size" with ``plot area" in this sentence, with the plot size ($20\times20$ m) being clarified in the followed parentheses. The revised sentence is:}

\textbf{Lines 123--125: \textcolor{blue}{``Field surveys were conducted to collect species richness samples in 2016 and 2017 for the two regions, with a sampling \underline{plot area of 400 m$^2$ (20 m $\times$ 20 m)} for each surveying location."}}

\textbf{The same change has also been applied to Table 1:}

\begin{table}[H]
\taburulecolor{blue}
\captionsetup{font=normalsize}
\caption*{\textcolor{blue}{Table 1: Information summary of the plant species richness samples collected in field observations.}}
{\color{blue}
\begin{tabularx}{\textwidth}{l l l}
\toprule
\textbf{}	& \textbf{Southern Tablelands}	& \textbf{Snowy Mountains}\\
\midrule
Number of Samples	 & 44 & 29\\
Sampling Time		& Feb 19, 2017 $\sim$ Dec 07, 2017 & Feb 24, 2016 $\sim$ Dec 13, 2017\\
\underline{Plot Area}		& \underline{400 m$^2$ (20 m $\times$ 20 m)} & \underline{400 m$^2$ (20 m $\times$ 20 m)}\\
Geo-extent		& \begin{tabular}[c]{@{}l@{}}34°12'26''--34°39'07''S\\ 150°05'57''--150°40'51''E\end{tabular} & \begin{tabular}[c]{@{}l@{}}35°43'58''--36°16'30''S\\ 148°23'16''--148°39'02''E\end{tabular}\\
\bottomrule
\end{tabularx}}
\end{table}

\bigbreak

- Sections 2.3 and 2.4: It seems that one of the objectives of the work was to test different feature extraction procedures (PCA, CCA, and PLS) and regression models (OLSR, GPR, and KRR) for predicting biodiversity. Nothing is mentioned in objectives. In Lines 88-89, considering the second objective, it is difficult to detect the best DESIS bands for this purpose with transformed data. Feature selection instead of feature extraction is more appropriate for this purpose.

\textbf{Re: Thanks for the valuable comment! As pointed out by the Reviewer, the main objective of our study is to test and compare several combinations of feature extraction procedures and regression models in predicting plant species richness from DESIS hyperspectral data. In order to clarify this objective, we have modified the title of this work. Relevant statements have been added in the Abstract, Introduction, and Conclusion sections. Detailed revisions are listed as follows:}

\textbf{(1) We have modified the title of the manuscript to the following in order to highlight the main objective of this work:}

\textbf{New Title: \textcolor{blue}{``Plant Species Richness Prediction from DESIS Hyperspectral Data: A Comparison Study on Feature Extraction Procedures and Regression Models"}}

\textbf{(2) In the Abstract section, the following sentence has been added to clarify the feature extraction procedures and regression models being tested in our study:}

\textbf{In Abstract: \textcolor{blue}{``We tested and compared the effectiveness of Principal Component Analysis (PCA), Canonical Correlation Analysis (CCA), and Partial Least Squares analysis (PLS) for feature extraction, and Ordinary Least Squares Regression (OLSR), Kernel Ridge Regression (KRR), and Gaussian Process Regression (GPR) for regression"}}

\textbf{In the revised manuscript, we have added some explanations on the merit of feature extract as compared with feature selection. The following sentences have been added in the Discussions section:}

\textbf{Lines 424--434: \textcolor{blue}{``Obtaining informative features from hyperspectral data is important to the success of subsequent interference of plant species richness. In previous studies, features have been primarily selected as a subset of the original bands, or as spectral indices computed from a subset of the original bands (e.g., \cite{malhi2020synergetic}, \cite{peng2018assessment}, and \cite{wang2016seasonal}). The bands or indices are often selected based on our \emph{a priori} knowledge of the spectral properties, such as absorption features of biochemical contents. Though selected features usually offer good explainability, it means we have to discard information in unselected bands. Considering the large number of bands in hyperspectral data, many of them would be discarded as the high collinearity of hyperspectral data often requires a considerable reduction of dimensionality. In contrast, the feature extraction approach, as adopted in this work, makes use of the information in all original bands by transforming them into a new feature space of lower and non-collinear dimensionality."}}

\bigbreak

- Section 2.3: Please, be clear on the input data for PCA, CCA, and PLS.

\textbf{Re: Thanks for the helpful suggestion! In the revised manuscript, we have improved the following sentence in order to clarify the input and output for PCA, CCA, and PLS:}

\textbf{Lines 192--195: \textcolor{blue}{``... \underline{the input data} for the transformation is $\mathbf{X}$, which is a $n\times m$ matrix consisting of the original spectra, with $n$ being the number of observed spectra and $m$ being the number of spectral bands; \underline{the output} of the transformation is $\mathbf{T}=[{\bm{t}}_1,{\bm{t}}_2, \cdots, {\bm{t}}_k]$, which is a $n\times k$ matrix consisting of $k$ components of $\mathbf{X}$ ..."}}

\bigbreak

- Section 2.4: Please, be clear on the input data used for each of the three regression models.

\textbf{Re: As suggested, we have improved relevant sentences in Section 2.4 in order to clarify the input data for each of the three regression models. Details revisions are listed below:}

\textbf{(1) For the Ordinary Least Squares Regression (OLSR) method:}

\textbf{Lines 216--217: \textcolor{blue}{``With the transformed components $\left \{ \bm{t}_i \right \}_{i=1}^n$ as \underline{input data}, the optimal set of model parameters, $\bm{b}^*$, can be found by solving the following optimisation problem ..."}}

\textbf{(2) For the Kernel Ridge Regression (KRR) method:}

\textbf{Lines 232--234: \textcolor{blue}{``The \underline{input data} for Eq. \ref{eq:krr} are the transformed components $\left \{ \bm{t}_i \right \}_{i=1}^n$. Solving Eq. \ref{eq:krr} does not involve calculating $\varphi(\bm{t}_i)$. Instead, it only requires computation of the inner product $k(\bm{t}_i, \bm{t}_j) = \varphi(\bm{t}_i)\varphi(\bm{t}_j)$, where $\bm{t}_i$ and $\bm{t}_j$ are pairs from the \underline{input data} $\left \{ \bm{t}_i \right \}_{i=1}^n$."}}

\textbf{(3) For the Gaussian Process Regression (GPR) method:}

\textbf{Lines 248--250: \textcolor{blue}{``The \underline{input data} for Eq. \ref{eq:gp} are the transformed components $\left \{ \bm{t}_i \right \}_{i=1}^n$. The covariance function $k(\bm{t}, \bm{t}')$ for GPR is set in the same way as that for KRR (Eq. \ref{eq:kernel_function}), i.e., $k(\bm{t}, \bm{t}')=k(\bm{t}_i, \bm{t}_j)$ where $\bm{t}_i$ and $\bm{t}_j$ are pairs from the \underline{input data} $\left \{ \bm{t}_i \right \}_{i=1}^n$."}}

\textbf{Many thanks for the valuable suggestion!}

\bigbreak

- Figure 6: Is very difficult to understand this figure. As presented, it does not add. Is there a better type of graphical representation?

\textbf{Re: We agree that the 3D representation of this figure was confusing. Thanks for pointing out this issue. In the revised manuscript, we have replaced it with a 2D representation. We hope this new figure, as shown in the following, is clear to readers:}

\begin{figure}[H]
\centering
\captionsetup{font=normalsize}
\includegraphics[width=15.2cm]{figures/kernel_params.jpg}
\caption*{\textcolor{blue}{Figure 6: Selection of kernel parameters $\sigma$, $l$, and $\delta$ based on grid search for Kernel Ridge Regression (KRR). The best performing combinations of kernel parameters are circled in black.}}
\end{figure}

\bigbreak

- Tables 2 and 3 summarizes the main objective of the work: test of different feature extraction approaches and regression models to predict species richness. The title of the work should be modified to reflect it.

\textbf{Re: We would like to thank the Reviewer for the insightful suggestion. In order to highlight the main objective of this work, we have modified the title in the revised manuscript. The new title of the manuscript is:}

\textbf{New Title: \textcolor{blue}{``Plant Species Richness Prediction from DESIS Hyperspectral Data: A Comparison Study on Feature Extraction Procedures and Regression Models"}}

\bigbreak

- Line 330: what is "a more stable basis"?

\textbf{Re: We have rephrased this sentence to make it clearer to readers. Thanks! The revised sentence is:}

\textbf{Lines 295--296: \textcolor{blue}{``Spaceborne multispectral imagery such as Sentinel-2 is \underline{more readily} \underline{available than hyperspectral}."}}

\bigbreak

- Sections 3.6 and 3.7 could migrate into a new Discussion section.

\textbf{Re: Thanks for the valuable suggestion. In the revised manuscript, we have created a new Discussions section. As suggested, Sections 3.6 and 3.7 (now indexed as Sections 4.2 and 4.3 in the revised manuscript) have been migrated to the Discussions section.}

\pagebreak

\textbf{\underline{Response to Reviewer 4's comments:}}

Reviewer 4: This paper evaluated the potential of the DESIS hyperspectral remotely sensed data from the ISS for mapping vascular plant species diversity in two sites in NSW, Australia. The topic is of high interest and importance in remote sensing. However, the analysis of this study is quite simple. There are a lot more analyses they can do. Here are my suggestions for revision.

\textbf{Re: Thank you very much for your careful review, and the insightful comments and suggestions. These comments and suggestions are highly valuable for us to improve this work. We have carefully revised the manuscript, with detailed revisions being listed below point by point in bold type font. Revised sentences are coloured in blue in this response letter, and highlighted in yellow background in the revised manuscript.}

\bigbreak

(1) There is no need to put some much math for PCA, CCA, and PLS in the manuscript as these math can be easily found in stats books. Nobody is really doing these analysis based on the math provide here, but using statistical packages to accomplish the analysis. The authors only need to describe how these transformation works in easy to understand plain language, and the difference among them in the description,

\textbf{Re: We would like to thank the Reviewer for the insightful suggestion. We agree with the Reviewer that it is common that statistical packages are being used for these analyses. Therefore, in the revised manuscript we have deleted the following paragraph where the mathematical procedure for computing PCA, CCA, and PLS was described:}

\textbf{Deleted: \textcolor{blue}{``The way in which PCA, CCA, and PLS compute the components $\left \{{\bm{t}}_i \right \}_{i=1}^{k}$ can be written as:
\begin{equation*}
\begin{split}
\arg\max_{{\bm{w}}_i} & \quad f({\bm{w}}_i), \\
{\rm{s.t.}} & \quad \left\| {\bm{w}}_i \right\| = 1, \\
& \quad {\bm{w}}_i^{\rm{T}}\mathbf{X}^{\rm{T}}{\mathbf{X}\bm{w}}_j = 0, \quad {\rm{for}} \quad j=1, \dots, i-1, \quad if \quad i > 1,
\end{split}
\end{equation*}
where $f({\bm{w}}_i)$ equals ${\rm{var}}(\mathbf{X}{\bm{w}}_i)$, ${\rm{corr}}(\mathbf{X}{\bm{w}}_i,\bm{y})$, and ${\rm{cov}}(\mathbf{X}{\bm{w}}_i,\bm{y})$ for PCA, CCA, and PLS, respectively. The components are computed iteratively from the first to the $k$th component by solving the above optimisation problem under two constraints. The first constraint in Eq. 1 limits ${\bm{w}}_i$ to be a unit vector, while the second constraint orthogonalises the current component ${\bm{t}}_i=\mathbf{X}{\bm{w}}_i$ with each of the previous components $\left \{ {\bm{t}}_j={\mathbf{X}\bm{w}}_j \right \} _{j=1}^{(i-1)}$ (this constraint does not apply to the computation of the first component ${\bm{t}}_1$)."}}

\textbf{Many thanks for the helpful comment!}

\bigbreak

(2) The number of species is just one of many biodiversity measurements. There are many other biodiversity measurements the authors should explore with these data. I also suggest that the authors separate the overstory diversity from the understory.

\textbf{Re: We would like to thank the Reviewer for the important comment. As pointed out by the Reviewer, species richness is just one of many variables to describe plant biodiversity. In this work, we have been focused on species richness only. In the revised manuscript, we have modified the title in order to clarify this:}

\textbf{New Title: \textcolor{blue}{``Plant \underline{Species Richness} Prediction from DESIS Hyperspectral Data: A Comparison Study on Feature Extraction Procedures and Regression Models"}}

\textbf{We agree with the Reviewer that separating the overstory diversity from the understory is an important topic to explore. Potentially tree richness and understory richness could be modelled separately, and then combined to get the total richness. Unfortunately, the data set used in our this work does not have information on which strata the observed species come from. In the revised manuscript, we have noted that it is worth exploring richness for different strata, with the following sentences having been added in the Discussions section:}

\textbf{Lines 492--497: \textcolor{blue}{``Moreover, though the data set used in this work does not have information on which strata the observed species come from, it is worth splitting out richness for different strata in future field surveys. With strata information on record, we might be able to model tree richness and understory richness separately, and then combine them once predicted to get total richness."}}

\bigbreak

(3) Figure 9 is an incomplete picture of the importance of the bands for biodiversity mapping. There are other components that the bands contribute to the regression results. I suggest using the vector length of importance values of each band to all components used in the regression weighted by its partial correlation coefficients as a measure for the importance of the band.

\textbf{Re: We would like to thank the Reviewer for the insightful suggestion. We agree that taking all components into consideration will provide a more comprehensive assessment of band importance. As suggested, we have revised the method for band importance analysis. In the revised manuscript, the vector length of contribution values of each band to all components used in the regression weighted by the partial correlation coefficients has been employed as the importance index of the band. The following subsection has been inserted in order to describe the method:}

\textbf{Lines 280--293:}

\subsection*{\textcolor{blue}{``\textbf{2.7 Band Importance Analysis}}}

\textcolor{blue}{\textbf{The DESIS data consist of spectral measurements over the visible and near-infrared bands from 400 nm to 1000 nm. Importance analysis was conducted in order to analyse which spectral bands provide more explanatory power than others in predicting plant species richness. We used the vector length of contribution values of each band to all components used in the regression weighted by the partial correlation coefficients as the importance index of the band:
\begin{linenomath*}
\begin{equation*}
I_{i}=\sqrt{\sum_{j=1}^{k}(w_{i,j}\cdot p_{j})^{2}},
\end{equation*}
\end{linenomath*}
where $I_{i}$ is the importance index for the $i$th band; $w_{i,j}$ is the $(i,j)$th element of the weight matrix $\mathbf{W}$ in Eq. \ref{eq:transformation}, representing the contribution of the $i$th band to the $j$th component; $p_{j}$ is the partial correlation coefficient of the $j$th component with the target variable of species richness; $k$ is the number of components used in regression. In our study, the importance indices $ I_{i}$ are normalised to relative values $\tilde{I}_{i}$ with sum over all bands equal to one:
\begin{linenomath*}
\begin{equation*}
\tilde{I}_{i} = \frac{I_{i}}{\sum_{i=1}^{m}I_{i}},
\end{equation*}
\end{linenomath*}
where $m$ is the number of spectral bands."}}

\textbf{In addition to the above added description, we have also updated the band importance figure in the Results section based on the new method. The updated figure is:}

\begin{figure}[H]
\centering
\includegraphics[width=10.5cm]{figures/sensitivity_new.jpg}
\captionsetup{font=footnotesize}
\caption*{\textcolor{blue}{Figure 10: Relative importance analysis for the DESIS bands in predicting plant species richness with spectral features being extracted by (a) Principal Component Analysis (PCA), (b) Canonical Correlation Analysis (CCA), and (c) Partial Least Squares analysis (PLS).}}
\end{figure}

\bigbreak

(4) Figure 6 is confusing. Please consider improve its readability.

\textbf{Re: We agree that the 3D representation of this figure was confusing. Thanks for pointing out this issue! In the revised manuscript, we have replaced the 3D figure with a 2D representation. We hope this new figure, as shown in the following, is clear to readers:}

\begin{figure}[H]
\centering
\captionsetup{font=normalsize}
\includegraphics[width=15.2cm]{figures/kernel_params.jpg}
\caption*{\textcolor{blue}{Figure 6: Selection of kernel parameters $\sigma$, $l$, and $\delta$ based on grid search for Kernel Ridge Regression (KRR). The best performing combinations of kernel parameters are circled in black.}}
\end{figure}

\textbf{Many thanks for the helpful comment!}

\pagebreak

\textbf{\underline{Response to Reviewer 5's comments:}}

Reviewer 5: This study is very timely and important. As much awaited new hyperspectral satellite missions such as DESIS have been launched, new research is needed to better understand the opportunities and limitations of these data in biodiversity monitoring in different climatic biomes and geographic regions. This study focusing on southeastern Australia ecosystems makes an important contribution in this direction and generates interesting results that could be compared to other regions in the future studies in Australia and elsewhere. The methodology is well described and well executed and the study provides a discussion of limitations.

I recommend this study to be considered for publication, but there are a few aspects of discussion of the study's results that need revision:

\textbf{Re: Thank you very much for your careful review, positive comments, and helpful suggestions. These comments and suggestions are highly valuable for us to improve this work. We have carefully revised the manuscript, with detailed revisions being listed below point by point in bold type font. Revised sentences are coloured in blue in this response letter, and highlighted in yellow background in the revised manuscript.}

\bigbreak

- Section 3.1 is written in a way that makes it more appropriate to Methods than to Resutls and Discussion. When Results and Discussion are combined in studies, it is often challenging to give enough room for actual discussion, and when information that should be in Methods is also added, it takes away from the interpretation. I would suggest separating the information out so that methodology in 3.1 has an appropriate place in Methods (add new subsection(s) there) while this section strictly discusses results and compares them to the literature with an informative discussion/syntehsis.

\textbf{Re: We would like to thank the Reviewer for pointing out this issue. As suggested, we have separated out the methodology-related materials from Section 3.1 (now indexed as Section 3.2 in the revised manuscript), and grouped them into a newly created Subsection (Section 2.5) in Methods. The new subsection is:}

\textbf{Lines 256--268:}

\subsection*{\textcolor{blue}{``\textbf{2.5 Determination of Hyperparameters}}}

\textcolor{blue}{\textbf{Hyperparameters that need to be pre-set included the number of components $k$ in the dimensionality reduction methods PCA, CCA, and PLS, and the kernel parameters $\sigma$, $l$, and $\delta$ in the non-linear regression method KRR.}}

\textcolor{blue}{\textbf{The number of components $k$ determines how much information to retain after dimensionality reduction. An optimal selection of $k$ is able to reduce data redundancy without excessively discarding useful information in the original DESIS spectra. In this study, we tested different $k$ values ranging from 1 to 10. The optimal $k$ value was selected based on the accuracy of species richness prediction, and the amount of variance in the spectral data that the retained components could explain.}}

\textcolor{blue}{\textbf{The tunable hyperparameters $\sigma$, $l$, and $\delta$ for the kernel function define the non-linearity structure of the regression model KRR. These kernel parameters were selected based on grid search. A grid of values was tested with each parameter varying from $10^{-5}$ to $10^{5}$ on a logarithmic scale. The combination of $\sigma$, $l$, and $\delta$ that produced the best performance in species richness prediction was selected."}}

\textbf{We have carefully checked sentences in other parts of the Results section. Materials that are more relevant to methodology than results have now been grouped into newly created subsections (i.e., Sections 2.7 and 2.8 in the revised manuscript) under the Materials and Methods section. Moving the methodology-related materials out of the Results section has created room for us to focus more on describing and discussing the results. As suggested, we have expanded the Results section in order to discuss the results more comprehensively and compare them to the literature in more detail. The added result descriptions and discussions are highlighted in yellow in the revised manuscript. Many thanks for the insightful comment!}

\bigbreak

- Similarly, check other subsections of Section 3 to avoid Methods language. For example the first sentence of 3.2 should be in Methods; here in 3.2 instead the text could be condensed and say more straightforwardly: " The assessment of different dimensionality reduction and regression methods (Table 2) should that .. the best results was achieved with a combination of PLS etc etc"

\textbf{Re: We would like to thank the Reviewer for the helpful suggestion. In the revised manuscript, we have moved the first sentence of Section 3.2 (now indexed as Section 3.3 in the revised manuscript) to the Materials and Methods section. The moved sentence and its new location is:}

\textbf{Lines 277--279: \textcolor{blue}{``Results with different feature extraction procedures (PCA, CCA, and PLS) and regression models (OLSR, KRR, and GPR) were computed and compared."}}

\textbf{Meanwhile, sentences at the beginning of Section 3.2 (now indexed as Section 3.3) have been condensed and improved as per the Reviewer's suggestion. The revised sentence is:}

\textbf{Lines 344--347: \textcolor{blue}{``The assessment of different dimensionality reduction and regression methods (Table 3) showed that, for the Southern Tablelands region, the best result was achieved with a combination of PLS for dimensionality reduction and GPR for regression, with $r$ being 0.76 and RMSE being 5.89."}}

\bigbreak

- One of the most interesting and important results of this study is well summarized in the Abstract: "Relative importance analysis for the DESIS spectral bands showed that the red-edge, red, and blue spectral regions were more important for predicting plant species richness than the green bands and the near-infrared bands beyond red-edge." However, there is relatively little discussion of it in the Results and Discussion section which makes this part somewhat unfinished in terms of understanding the implications of this findings.

\textbf{Re: We would like to thank the Reviewer for the highly helpful comment. In the revised manuscript, we have carefully revised the band importance section. The discussion on band importance result has been enhanced with citations of previous literature using hyperspectral data. Interpretation of the result has been revisited with more explanation being added based on the cited literature. The revised section for band importance analysis is:}

\textbf{Lines 379--397:}

\subsection*{\textbf{\textcolor{blue}{``3.5. The Relative Importance of Spectral Bands}}}

\textbf{\textcolor{blue}{The relative importance of DESIS bands in predicting plant species richness is shown in Fig. \ref{fig:relative}, with the aim to analyse which parts of the spectrum had the most explanatory power. Subplots \ref{fig:relative}a, b, and c display the results with PCA, CCA, and PLS being used as the feature extraction procedure, respectively. From these subplots, it was observed that bands in the red-edge spectral region of approx. 700 $\sim$ 720 nm showed the highest importance. This observation might be supported by literature that the red-edge is an important spectral region for vegetation mapping as it is closely related to biological variables such as leaf area index \citep{delegido2013red}, plant vigour \citep{boochs1990shape}, and biochemical contents \citep{mutanga2007red}. Followed by the red-edge, the visible range of approx. 400 $\sim$ 700 nm also showed high importance. The importance of visible bands in plant species richness prediction might be justified by the fact that, this portion of the spectrum, especially bands in red and blue, is the major leaf pigment absorption range. It is sensitive to mainly chlorophyll a and b contents, according to the sensitivity analysis result reported in \cite{zhao2014earlya, zhao2014earlyb}. Though less important than the red-edge and visible regions, the near-infrared region with wavelengths longer than 720 nm also showed some explanatory power. This indicated that the near-infrared region also provided contributory information in predicting plant species richness, as this portion of the spectrum, often characterised by high reflectance for vegetation, is sensitive to leaf thickness \citep{zhao2014earlyb} and the amount, arrangement, and inclination of leaves in the canopy \citep{knipling1970physical}."}}

\begin{figure}[htb!]
\centering
\includegraphics[width=10cm]{figures/sensitivity_new.jpg}
\captionsetup{font=footnotesize}
\caption*{\textcolor{blue}{Figure 10: Relative importance analysis for the DESIS bands in predicting plant species richness with spectral features being extracted by (a) Principal Component Analysis (PCA), (b) Canonical Correlation Analysis (CCA), and (c) Partial Least Squares analysis (PLS).}}
\end{figure}

\bigbreak

- The paper should one or a couple of paragraph to discuss "WHY" this may be the case - certain spectral regions more important than ohters, based on the knowledge of vegetation physiology and previous literature using hyperspectral data. To build this discussion, one would need to look back to studies using field and airborne spectroscopy - there has been a lot of relevant work in the past on the role of different pigments in photosynthetic absorption and their narrowband spectra; also the mechanistic basis behind popular vegetation indices, etc, and citing the appropriate studies.

\textbf{Re: We agree with the Reviewer that it is necessary to cite previous spectroscopy literature in order to enhance discussion of the results. We have carefully revised the Results section with improved discussions being added based on the cited literature. Detailed revisions are listed below:}

\textbf{(1) For the band importance results, more explanations have been added in the revised manuscript from a spectroscopical point of view. Please refer to our response to the previous comment for the revised section.}

\textbf{(2) A new subsection has been added to the Results section, in order to show the reflectance differences between low, intermediate and high species richness plots. The results have been explained from a spectroscopical point of view, with supporting materials from the literature. This new section is:}

\textbf{Lines 309--323:}

\subsection*{\textcolor{blue}{``\textbf{3.1. Spectral Reflectance Differences Between Species Richness Classes}}}

\textcolor{blue}{\textbf{The blue, green and red curves in Fig. \ref{fig:different_richness} show the DESIS spectra averaged over ground sampling plots with species richness falling into the low, intermediate, and high tertiles, respectively. Results for the Southern Tablelands and Snowy Mountains regions are displayed in Figs \ref{fig:different_richness}a and b, respectively. For each region, it was observed that plots of higher richness showed a lower reflectance in the visible range of $400\sim680$ nm. Considering that major absorption features of chlorophyll are located within the visible region \citep{zhao2014earlya}, the lower reflectance in this spectral portion might indicate a higher concentration of chlorophyll. It was also observed that plots of higher richness showed a higher reflectance in the near-infrared plateau of $780\sim1000$ nm and a steeper red edge between $680\sim780$ nm, which might suggest a larger Leaf Area Index (LAI) \citep{delegido2013red} and a greater vegetation vigor \citep{boochs1990shape} for those plots. On the basis of these observations, the spectral shape of high richness plots, as compared with spectra of intermediate and low richness plots, may imply a generally richer vegetation. This is consistent with findings reported in literature that high species richness enhances primary productivity \citep{wang2016seasonal, grace2016integrative} and biomass \citep{malhi2020synergetic, tilman1997influence}."}}

\begin{figure}[H]
\centering
\captionsetup{font=footnotesize}
\includegraphics[width=8.5cm]{figures/different_richness.jpg}
\caption*{\textcolor{blue}{Figure 4: Average DESIS reflectance spectra calculated from field sample plots with low, intermediate, and high species richness for the (a) Southern Tablelands and (b) Snowy Mountains regions.}}
\end{figure}

\textbf{Many thanks for the valuable suggestion!}

\bigbreak

- It is commendable that this study included a Limitations section; however, one important item is not in it and should be discussed - the uncertainty associated with spatial resolution of DESIS. A plot size of 400 m2 is not likely to perfectly match a DESIS pixel even in case of a perfect georegistration. Please add a few sentences to discuss the uncertainty associated with this and its potential implications or the future research needs that might stem out of it.

\textbf{Re: We would like to thank the Reviewer for this important suggestion. We agree that the uncertainty associated with pixel/plot size is worth for discussion. As pointed out by the Reviewer, there is a mismatch between the DESIS pixel size and the ground plot area. Potential inaccuracies in geo-registration of DESIS images and in geo-positioning measurements during field surveys may also result in geo-mismatch between pixels and ground plots. They are worth attention and exploration in future research. In the revised manuscript, we have inserted the following new paragraph in the Limitations section to add discussions on the uncertainty issue and suggestions for future research:}

\textbf{Lines 498--508: \textcolor{blue}{``It is important to note that the DESIS pixel size ($30\times30$ m) does not match exactly with the plot area of ground species richness samples ($400\;\text{m}^{2}=20\times20\;\text{m}$). Though richness measurements could be scaled to a larger or smaller plot area using an assumed power relationship ($S=cA^{z}$) between species richness ($S$) and plot area ($A$) \citep{rosenzweig1995species}, the location-specific power parameter ($z$) is often hard to be accurately determined without adequate knowledge about the experiment site. It is suggested that, in future field campaigns, it is worthwhile to gather information on the richness-area relationship, in order to facilitate accurate up- and down-scaling of plot areas. Potential inaccuracies in geo-registration of DESIS images and in geo-positioning measurements during field surveys may also result in geo-mismatch between pixels and ground plots. Better geo-registration and geo-positioning accuracies would help reduce uncertainties in predicting species richness in future works."}}

==> response_letter_second_round.tex <==
\begin{center}
\large
\textbf{Response to Reviewers' Comments}
\end{center}

\begin{center}
Ms. Ref. No.: PHOTO-D-22-00486

ISPRS Journal of Photogrammetry and Remote Sensing
\end{center}

\bigbreak

\begin{flushleft}
\textbf{Dear Editor:}
\end{flushleft}

\textbf{Many thanks for your time handling our manuscript! We appreciate the insightful comments and suggestions from the Reviewers which have allowed us to improve the quality of our manuscript further. We have carefully revised the manuscript, with our responses to Reviewers' comments being detailed below point by point in bold type font. Revised sentences are coloured in blue in this response letter, and highlighted in yellow background in the revised manuscript.}

\bigbreak

\textbf{\underline{Response to Reviewer 1's comments:}}

Reviewer 1: Thanks very much for revising the manuscript. This is a much-improved version. I am satisfied with the implemented modifications in the text by the authors. Therefore, I recommend publication. However, there is space to polish the text in Abstract during proofreading replacing expressions like "strongest results".

\textbf{Re: We would like to thank the Reviewer for the positive comments. In the revised manuscript, we have replaced ``strongest results" in the Abstract with the ``The best prediction results". Many thanks for the helpful suggestion!}

\bigbreak

\textbf{\underline{Response to Reviewer 4's comments:}}

Reviewer 4: This paper used DESIS hyperspectral imagery to map plant species richness at two sites in Australia, and compared the results from the hyperspectral imagery with the broad band imagery from Sentinel-2. They first transformed the data with PCA, CCA and PLS and then compared three regression analyses, OLSR, KRR and GPR. They found that red-edge, red and blue spectral regions were more important than other bands in mapping species richness. The topic is of high interest to readers of remote sensing. However, the work is exceedingly long, but missing key methodologies to examine the potential of DESIS in mapping species riches. Thus I suggest another round of major revision (Sorry!) as I know you already went through a round of major revision.

\textbf{Re: We appreciate the important comments and suggestions from the Reviewer. These comments and suggestions are highly valuable for us to improve this work further. We have carefully examined and revised the manuscript. As suggested by the Reviewer, we have added a key regression method (Random Forest) which has shown superior performance. We have also shortened the manuscript by removing the Ordinary Least Squares Regression (OLSR) as the method is similar to others adopted in our study. Detailed revisions are listed below point by point in bold type font. Revised sentences are coloured in blue in this response letter, and highlighted in yellow background in the revised manuscript.}

\bigbreak

1. The three data transformation are more or less the same, redundancy reduction. In fact, both CCA and PLS are different from PCA and CCA and PLS requires a set of dependent variables in the data transformation. I would not consider PLS and CCA as data transformation but only PCA is. There is no need to have all three of them included here as render similar effect on the data as one can be seen in Figure 10. Moreover, CCA and PLS already provide correlation analysis, as I understand. Why do you need to use the transformed inputs to other regression algorithms? The authors used the transformed data as inputs to another set of regression analysis tools, OLSR, KRR and GPR . Again these regression analysis tools are similar by and large as can be seen in Figure 6. I suggest authors to drop OLSR and KRR, but include a few different machine learning algorithms, as well as their ensemble to explore the potential of DESIS data in mapping species richness. Some machine learning algorithms, such as the Random Forest, also provide the variable importance score.

\textbf{Re: We agree with the Reviewer that, with a range of advanced machine learning algorithms, we can better explore the potential of DESIS data in mapping species richness. As suggested, we have included Random Forest Regression (RFR) in our revised manuscript. In addition to RFR as an ensemble approach, we have kept Kernel Ridge Regression (KRR) and Gaussian Process Regression (GPR) in the revised manuscript, considering that these two algorithms belong respectively to the deterministic and Bayesian categories. We hope the three algorithms adopted in our work would cover a range of regression techniques allowing a broad assessment of the ability of DESIS instrument in predicting plant species richness. We have removed the Ordinary Least Squares Regression in order to reduce the length of the manuscript. Detailed revisions are listed below:}

\textbf{(1) In Subsection 2.4, the following description of Random Forest Regression has been added:}

\textbf{Lines 248--256:} \textcolor{blue}{``In addition to KRR and GPR that are  respectively belong to the deterministic and Bayesian regression categories, we also tested the ensemble method of RFR. A random forest combines a number of decision tree regressors and takes the average regression result over all trees as the final estimate. Due to the ensemble structure, RFR tends to produce robust regression results with high resistance to overfitting and data noise. The training of a random forest regressor minimises the following optimization function:
\begin{equation*}
\arg\min_{\bm{\theta}_{j}} \quad  \dfrac{1}{d}\sum_{j=1}^{d} \sum_{i=1}^{n} \left[h(\bm{t}_i;\bm{\theta}_{j})-y_i \right] ^2,
\end{equation*}
where $h(\cdot)$ is the decision tree regressor with $\bm{\theta}_{j}$ being the parameters of the $j$th tree; $d$ is the number of decision trees, which was set to 100 in this study."}

\textbf{(2) In Subsection 2.4, the following description of Ordinary Least Squares Regression has been deleted:}

\textbf{Deleted:} \textcolor{blue}{``Then with OLSR, a linear model with parameters $\bm{b}$ can be built to minimise the sum of squared errors between the model-predicted species richness $\bm{t}_i^{\text{T}}\bm{b}$ and ground-truth species richness $y_i$. With the transformed components $\left \{ \bm{t}_i \right \}_{i=1}^n$ as input data, the optimal set of model parameters, $\bm{b}^*$, can be found by solving the following optimisation problem:
\begin{equation*}
\arg\min_{\bm{b}} \sum_{i=1}^{n} (\bm{t}_i^{\text{T}}\bm{b}-y_i)^2.
\end{equation*}
After the optimal $\bm{b}^*$ is determined, for a new spectrum $\bm{x}$ with its extracted components $\bm{t}$, the predicted species richness is $\hat{y}=\bm{t}^{\text{T}}\bm{b}^*$."}

\textbf{(3) In Subsection 3.3, Tables 3 and 4 have been updated, with results for Ordinary Least Squares Regression being deleted and those for Random Forest Regression being added. Text descriptions of the results have also been updated in Subsection 3.3. The updated sentences are:}

\textbf{Lines 345--351:} \textcolor{blue}{``The assessment of different dimensionality reduction and regression methods (Table {\ref{tab:southern_tablelands}}) showed that, for the Southern Tablelands region, the best result was achieved with a combination of PLS for dimensionality reduction and GPR for regression, with $r$ being 0.76 and RMSE being 5.89. Results with PLS as the dimensionality reduction method performed better than those with PCA and CCA. The PLS-based models achieved $0.75\sim 0.76$ for $r$ and $5.92\sim 6.00$ for RMSE, respectively, better than the PCA-based models with $0.70\sim 0.71$ for $r$ and $5.99 \sim 6.02$ for RMSE, and the CCA-based models with $0.69\sim 0.72$ for $r$ and $5.98 \sim 6.02$ for RMSE."}

\textbf{Lines 356--357:} \textcolor{blue}{``The best $r$ and RMSE were 0.68 and 5.95, respectively, achieved with a combination of PLS for dimensionality reduction and RFR for regression."}

\textbf{For dimensionality reduction, we have kept the three methods of PCA, CCA, and PLS, as they follow different criteria to reduce spectral dimensions. PCA aims to explain the maximum variance in the spectral data, CCA maximises the correlation between the variables, and PLS maximises the covariance.}

\textbf{Many thanks for the helpful suggestion!}

2. The conclusion that red-edge bands are among the most sensitive bands for species richness mapping is not supported by the data, particularly Figure 4, where one sees no difference in red-edge reflectance for plots with different species richness, it is the visible and near and mid-infrared bands that matter. The authors need to carefully examine the results here.

\textbf{Re: We would like to thank the Reviewer for this important suggestion. As pointed out by the Reviewer, the low, intermediate, and high species richness plots in Figure 4 showed similar values in the red-edge spectral region, while their red-edge slopes are different, which may explain the reason that red-edge bands are of high importance in plant species richness prediction. With careful examination of the result, we have added the following sentences in the revised manuscript, aiming to explain the high sensitivity in red-edge bands:}

\textbf{Lines 380--387:}  \textcolor{blue}{``From these subplots, it was observed that bands in the red-edge spectral region of approx. 700 $\sim$ 720 nm showed the highest importance. \textbf{This may suggest that the slope of the red-edge is an important spectral feature for plant species richness prediction, considering that the low, intermediate, and high species richness plots showed varied red-edge slopes in Fig. 4.} This observation might be supported by literature that the red-edge is a critical spectral region for vegetation mapping as it is closely related to biological variables such as leaf area index \citep{delegido2013red}, plant vigour \citep{boochs1990shape}, and biochemical contents \citep{mutanga2007red}."}

\textbf{Thanks for the valuable comment!}

\bigbreak
